Wind Flow Estimation in Thermal Sky Images for Sun Occlusion Prediction

Moving clouds affect the global solar irradiance that reaches the surface of the Earth. As a consequence, the amount of resources available to meet the energy demand in a smart grid powered using Photovoltaic (PV) systems depends on the shadows projected by passing clouds. This research introduces an algorithm for tracking clouds to predict Sun occlusion. Using thermal images of clouds, the algorithm is capable of estimating multiple wind velocity fields with different altitudes, velocity magnitudes and directions.

==> Wind%20Flow%20Estimation%20in%20Thermal%20Sky%20Images%20for%20Sun%20Occlusion%20Prediction%20(IEEE-PES-ISGT2021)-2/methods.tex <==
\section{Multiple Wind Velocity Field Estimation}

\subsection{Velocity Vectors Calculation}

\subsubsection{Beta Mixture Model}

Consider the temperatures $\bar{T}_{i,j}$ of a given image (by omitting superindex $k$). The distribution of the normalized temperatures can be approximated by a mixture of beta distributions $\bar{T} \sim Be ( \alpha_c, \beta_c )$ with the density function,
\begin{equation}
    \label{eq:beta_distribution}
    f \left( \bar{T}_{i,j} ; \alpha_c, \beta_c \right) = \frac{1}{\mathrm{B} \left( \alpha_c, \beta_c \right)} \cdot \bar{T}_{i,j}^{\alpha_c - 1} \cdot \left( 1 - \bar{T}_{i,j}\right)^{\beta_c - 1}, \quad \alpha_c, \beta_c > 0,
\end{equation}
where $\bar{T}_{i,j} \in (0, 1)$,  the beta function is $\mathrm{B} ( \alpha_c, \beta_c ) = [ \Gamma ( \alpha_c ) \Gamma ( \beta_c ) ] / [\Gamma ( \alpha_c + \beta_c ) ] $, and the gamma function is $\Gamma ( \alpha_c ) = ( \alpha_c - 1 ) !$.

The log-likelihood of the beta density function that we need to compute the expected complete data log-likelihood (CDLL) is,
\begin{equation}
    \log p \left( \bar{T}_{i,j}\mid \alpha_c, \beta_c \right) = \left( \alpha_c - 1 \right) \log \bar{T}_{i,j}+ \left( \beta_c - 1 \right) \log \left( 1 - \bar{T}_{i,j} \right)- \log \mathrm{B} \left(\alpha_c, \beta_c \right),
\end{equation}
and the CDLL in a mixture model is,
\begin{equation}\label{EM_likelihood}
   \mathcal{Q} \left( \boldsymbol{\theta}^{\left( t\right)}, \boldsymbol{\theta}^{\left(t - 1\right)}\right) = \sum_{i = 1}^M \sum_{j = 1}^N \sum_{c = 1}^C \gamma_{i,j,c} \log \pi_c + \sum_{i = 1}^M \sum_{j = 1}^N \sum_{c = 1}^C \gamma_{i,j,c}  \log p \left( \bar{T}_{i,j} \mid \boldsymbol{\theta}^{\left( t\right)} \right)
\end{equation}
where $\gamma_{i,j,c} \triangleq  p ( y_{i,j} = c \mid \bar{T}_{i,j}, \boldsymbol{\theta}^{(t - 1)} )$ is the responsibility of the cluster $c$ in the sample $i,j$ and $\boldsymbol{\theta}^{( t)} = \{\alpha_c^{\left( t\right)} , \beta_c^{( t)} \}$.

The parameters in the clustering of beta distributions can be directly computed applying the Expectation Maximization (EM) algorithm \cite{MURPHY2012}. In the E stage of the algorithm a prior is established and then, by using the likelihood function \eqref{EM_likelihood}, a posterior $\gamma_{i,j,c} = p(y_{i,j} = c \mid \bar{T}_{i,j}, \boldsymbol{\theta})$ can be assigned to each sample \cite{BISHOP2006}. In the M stage, the parameters $\alpha_c$ and $\beta_c$ of each cluster that maximize the log-likelihood are computed by gradient descent of the CDLL \cite{NOCEDAL2006}. The corresponding derivatives are,
\begin{equation}
    \begin{split}
        \frac{\partial \mathcal{L} \left( \boldsymbol{\theta} \right)}{\partial \alpha_c} &=  \sum_{i = 1}^M \sum_{j = 1}^N \sum_{c = 1}^C \gamma_{i,j,c} \frac{\partial}{\partial \alpha_c} \log p \left( \bar{T}_{i,j} \mid \alpha_c, \beta_c \right) \\
        &= \sum_{i = 1}^M \sum_{j = 1}^N \gamma_{i,j,c} \sum_{c = 1}^C \left[ \log \bar{T}_{i,j} - \psi \left( \alpha_c \right) + \psi \left( \alpha_c + \beta_c \right) \right], \\
        \frac{\partial \mathcal{L} \left( \boldsymbol{\theta}_c \right)}{\partial \beta_c} &= \sum_{i = 1}^M \sum_{j = 1}^N \sum_{c = 1}^C \gamma_{i,j,c} \left[
        \frac{\partial}{\partial \beta_c} \log p \left( \bar{T}_{i,j} \mid \alpha_c, \beta_c \right) \right] \\
        &= \sum_{i = 1}^M \sum_{j = 1}^N \gamma_{i,j,c} \sum_{c = 1}^C \left[ \log \left( - \bar{T}_{i,j} \right)- \psi \left( \beta_k \right) + \psi \left( \alpha_c + \beta_c \right) \right].
    \end{split}
\end{equation} 
where $\partial \mathrm{B} ( \alpha_c, \beta_c ) / \partial \alpha_c  = \mathrm{B} ( \alpha_c, \beta_c ) \cdot [ \psi ( \alpha_c ) - \psi ( \alpha_c + \beta_c ) ]$, and $\psi ( \cdot )$ is the digamma function, which is $\psi ( \alpha_c ) = \Gamma^\prime ( \alpha_c ) / \Gamma \left( \alpha_c \right)$.

The optimal priors are found by maximizing the CDLL with respect to $\pi_c$, constrained to $\sum_c\pi_c=1$. As a result, the optimal priors are
\begin{equation}
    \pi_c = \frac{1}{MN}\sum_{i = 1}^M \sum_{j = 1}^N \gamma_{i,j,c}.
\end{equation}

The cloud average heights in a frame are computed using the posterior probabilities $\gamma_{i,j,c}$ in a frame, but only in the pixels with a cloud,
\begin{equation}
    \hat{H}_c = \frac{\sum_{i,j} \gamma_{i,j,c} \cdot H_{i,j} \cdot \mathbb{I} \left( b_{i,j} = 1 \right)}{\sum_{i,j} \gamma_{i,j,c} \cdot \mathbb{I} \left( b_{i,j} = 1 \right)},
\end{equation}
where $\mathbb{I} \left( \cdot \right)$ is the indicator function. An image segmentation algorithm indicates which pixels belong to a cloud, so that $\mathbf{B} = \{ b_{i,j} \in \mathbb{B} \mid \forall i = 1, \ldots, M, \ \forall j = 1, \ldots, N \}$ is a binary image where 0 is a clear sky pixel, and 1 is a pixel belonging to a cloud \cite{TERREN2020c}. 

The performance of a Gamma Mixture Model and a BeMM were compared to infer the distribution of the temperatures and the heights. The BeMM of the temperature of the pixels was found to be better when identifying which pixels belong to the wind velocity layer.

\subsubsection{Weighted Lucas-Kanade}

%In current computer vision literature, there are three primary methods to estimate the motion of objects in a sequence of images: Lucas-Kanade \cite{LUCAS1981}, Horn-Schunk \cite{HORN1981}, and Farneb{\"a}ck \cite{FERNEBACK2003}. These three methods are based on the space-time partial derivatives between two consecutive frames. Taking a different disciplinary approach, the velocity field in experimental fluid dynamics is approximated applying research methods based on signal cross-correlation operated in the frequency domain \cite{ADRIAN2011}. 

The techniques to estimate the motion vectors in an image are sensitive to the intensity gradient of the pixels. We implemented a model that removes the gradient produced by the solar direct radiation, and atmospheric scattered radiation, both of which routinely appear on the images in the course of the year. A persistent model of the outdoor germanium window of the camera removes sporadic debris that appears in the images such as water stains or dust particles \cite{TERREN2020a}.

%A series of sequences of images with clouds flowing in different directions were simulated to cross-validate the set of parameters for each one of the mentioned methods. The investigation searched for a dense implementation of a motion vector method to approximate the dynamics of clouds. 

The most suitable method was found to be the Weighted Lucas-Kanande (WLK) \cite{SIMON2003}. The weights $\gamma_{i,j,c}$ are the posterior probabilities of the BeMM. Therefore, a pixel has a velocity vector for each cloud layer $c$ in a frame. The optimal window size, weighted least-squares regularization, and differential kernel amplitude are: $\mathcal{W} = 16 [ \mathrm{pixels}^2 ]$, $\tau = 1 \times 10^{-8}$, and $\sigma = 1$ respectively. The velocity components in the x-axis are ${\bf U}_c = \{ \text{u}_{i,j,c} \in \mathbb{R} \mid \forall i = 1, \ldots, M, \ \forall j = 1, \ldots, N \}$, and  the velocity components in the y-axis are ${\bf V}_c = \{ \text{v}_{i,j,c} \in \mathbb{R} \mid \forall i = 1, \ldots, M, \ \forall j = 1, \ldots, N \}$. The velocity vectors are in units of pixels per frame, but knowing the geometrical transformation of the frame, they can be transformed to meters per second \cite{TERREN2020a}. The geometric transformation is a function of the Sun's elevation and azimuth angles $\psi : \left( \varepsilon, \alpha \right) \mapsto \Delta \mathbf{x}_{i,j} $ in a frame, it defines the dimensions of a pixel at a given height $ \Delta \mathbf{X} = \{ \left(\Delta x, \Delta y \right)_{i,j} \mid\forall i = 1, \ldots, M, \ \forall j = 1, \ldots, N \}$. This transformation connects the x,y-axis coordinates system with the height, which is the z-axis. The relation holds even when the height is an approximation, since the components of velocity vectors are transformed with respect to the new coordinates system. The velocity vectors of each cloud layer are transformed such as,
\begin{equation}
    \label{eq:geometric_transformation}
    \begin{split}
        u_{i,j} &= \frac{\delta}{f_r}  \cdot \Delta x_{i,j} \sum_{c = 1}^C  \hat{H}_c \cdot \gamma_{i,j,c} \cdot \text{u}_{i,j,c}  \\
        v_{i,j} &= \frac{\delta}{f_r} \cdot \Delta y_{i,j} \sum_{c = 1}^C \hat{H}_c \cdot \gamma_{i,j,c} \cdot \text{v}_{i,j,c}
    \end{split}s
\end{equation}
where $f_r$ is the frame rate of the sequence of images, and $\delta$ is velocity vectors' scale in the WLK approximation.

\subsection{Velocity Vectors Selection}

In order to approximate the potential lines and streamlines of the wind velocity field in a frame, we propose to select the most consistent velocity vectors over a sequence of consecutive frames. The main problems with this approach are that as the vectors are selected over a sequence of images, the amount of vectors is expected to be large; also when optical flow is implemented in dense manner, it yields to noisy vectors. Because of this, we threshold the velocity vectors to reduce both the algorithm's computational burden and the variance of the noise.

\subsubsection{Velocity Vector Segmentation}

The pixel intensity difference between two consecutive frames is computed to find the pixels that show a change. The pixel normalized intensities that were used to compute the velocity vectors are ${\mathbf{I}} = \{ {i}_{i,j} \in \mathbb{R}^{[0, 2^8)} \mid \forall i = 1, \ldots, M, \ \forall j = 1, \ldots, N \}$. The root squared intensity normalized difference is,
\begin{equation}
    {d}_{i,j} =\frac{ \sqrt{\left({i}^{k - 1}_{i,j} - {i}^k_{i,j}\right)^2}}{\sum_{i,j}{ \sqrt{\left({i}^{k - 1}_{i,j} - {i}^k_{i,j}\right)^2}}}.
\end{equation}

Matrix ${\bf D}$ with normalized differentials $d_{i,j}$ is vectorized and sorted from the lowest to the highest, i.e., ${\mathbf{d}} = \mathrm{sort}(\mathrm{vec} ({\mathbf{D}} ))$. A vector $\bf r$ with the accumulated variance is computed as
\begin{equation}
    r_m = \left\{ \sum^m_{i = 1} {\bf d}_i \right\}^{N \cdot M}_{m = 1}.
\end{equation}
Then, vector $\mathbf{r}$ is reorganized and set in the original matrix form, defined as $\mathbf{R} = \{ r_{i,j} \in \mathbb{R}^{[0,1)} \mid \forall i = 1, \dots, M, \ \forall j = 1, \dots, N \}$. Finally, a threshold $\tau$ is applied
\begin{equation}
    \label{eq:threshold}
    b_{i,j} = 
    \begin{cases}
        1 \quad r_{i,j} \geq \tau \\
        0 \quad \mathrm{Otherwise},
    \end{cases}
\end{equation}
where  $\mathbf{B} \in \mathbb{B}$ is a binary image whose elements are 1 when a pixel is selected. The threshold velocity vectors in a frame $k$ are ${{\bf V}'}^{k} = \{ \mathbf{v}^k_{i,j}=\{u_{i,j}^k,v_{i,j}^k\}  \wedge b^k_{i,j} = 1 \mid \forall i = 1, \ldots M, \ \forall j = 1, \ldots, N \}$.

Based on the assumption that a cloud floating in the air follows a trajectory dictated by the wind velocity field, the wind velocity field is approximated using the segmented velocity vectors of $\ell$ last frames. Hence, the set of velocity vectors available to compute the wind velocity field are,
\begin{equation}
    \label{eq:dataset}
    \tilde{\mathbf{V}}^{k} = \left[ {\begin{array}{ccc}
       {{\bf V}'}^k \\
       \vdots \\
       {{\bf V}'}^{k - \ell} \\
      \end{array} } \right] \in \mathbb{R}^{2 \times N^k},
\end{equation}
the number of samples in $\tilde{\mathbf{V}}^k$ is $N^k$, this number is not the same in each frame $k$. 

\subsubsection{Velocity Vector and Height Distributions}

A velocity vector $\tilde{\mathbf{v}}_i$ (by omitting superindex $k$) in the set $\tilde{\mathbf{V}}^k = \{ \tilde{\mathbf{v}}^k_i \in \mathbb{R}^2 \mid \forall i = 1, \dots, N^k\}$ is assumed to belong to a cloud layer $c$. The probability of a vector to belong to a cloud layer $c$ is modelled as an independent normal random variable $\tilde{\mathbf{v}}_i \sim \mathcal{N}( \boldsymbol{\mu}_c, \boldsymbol{\Sigma}_c )$. The function of the multivariate normal distribution is,
\begin{equation}
    p \left( \tilde{\mathbf{v}}_i \mid  \boldsymbol{\mu}_c, \boldsymbol{\Sigma}_c \right) = \frac{\mathrm{e}^{\left\{ - \frac{1}{2} \left( \tilde{\mathbf{v}}_i - \boldsymbol{\mu}_c \right)^\top \boldsymbol{\Sigma}_c^{-1} \left( \tilde{\mathbf{v}}_i- \boldsymbol{\mu}_c \right) \right\}}}{\sqrt{ \left(2 \pi\right)^d \left| \boldsymbol{\Sigma}_c \right| }}.
\end{equation}
In the case when two cloud layers were detected, we propose to infer the probability distribution of velocity vectors' in each cloud layer with this model,
\begin{equation}
    p \left( \tilde{\mathbf{v}}_i \mid \boldsymbol{\Theta} \right) \propto p \left( \tilde{\mathbf{v}}_i \mid \boldsymbol{\mu}_1, \boldsymbol{\Sigma}_1 \right)^{\lambda_i} \cdot  p \left( \tilde{\mathbf{v}}_i  \mid \boldsymbol{\mu}_2, \boldsymbol{\Sigma}_2 \right)^{\left(1 - \lambda_i \right)},
\end{equation}
where $\boldsymbol{\Theta} = \{ \boldsymbol{\lambda}, \boldsymbol{\mu}_1, \boldsymbol{\Sigma}_1, \boldsymbol{\mu}_2, \boldsymbol{\Sigma}_2\}$, and $\lambda_i \in \{0, 1\}$.  $\lambda_{i,c}$ is defined as convex, considering that a velocity vector may belong to one or the other wind velocity layer, but no to both. Knowing the vectors that belong to the first cloud layer, the vectors that belong to the second cloud layer are also known, $\lambda_{i,2} = 1 - \lambda_{i,1}$. The lower bound of the data log-likelihood is found applying Jensen's inequality \cite{JENSE1906},
\begin{equation}
	\label{eq:velocity_vectors_distribution}
    \log p \left( \tilde{\mathbf{v}}_i \mid {\boldsymbol{\Theta}} \right) \propto \lambda_{i,1} \cdot \log p \left( \tilde{\mathbf{v}}_i \mid {\boldsymbol{\mu}}_1, {\boldsymbol{\Sigma}}_1 \right) + \lambda_{i,2} \cdot \log p \left( \tilde{\mathbf{v}}_i  \mid {\boldsymbol{\mu}}_2, {\boldsymbol{\Sigma}}_2 \right),
\end{equation}
so that the posterior distribution is a linear combination of the multivariate normal distributions.

The probabilistic model parameters are inferred using a fixed-point variation of the Iterated Conditional Modes (ICM) \cite{BESAG1986}. The algorithm begins by randomly assigning the velocity vectors to a cloud layer, $\lambda_{i,1} \sim \mathcal{U} ( 0, C - 1 )$. The parameters of velocity vector distributions, in Eq. \eqref{eq:velocity_vectors_distribution} that maximize the data log-likelihood are computed in the first step of the algorithm. These same parameters are used to initialize the inference of the parameters of the height distributions in the second step in Eq. \eqref{eq:height_distributions}. 

In the case of a multivariate normal distribution, the ICM algorithm is iteratively updates parameters. At iteration $t+1$, the means and covariances are,
\begin{equation}
    \label{eq:parameters_estimation}
    {\boldsymbol{\mu}}_c^{(t + 1)} = \frac{\sum_i \lambda_{i,c}^{(t)} \cdot \tilde{\mathbf{v}}_i }{\sum_i \lambda_{i,c}^{(t)}}; \ \ \
    {\boldsymbol{\Sigma}}_c^{(t + 1)} = \frac{\sum_{i} \lambda_{i,c}^{(t)} \cdot \left( \tilde{\mathbf{v}}_i  - {\boldsymbol{\mu}}_c^{(t + 1)} \right)^\top \left( {\mathbf{v}}_i  - \tilde{\boldsymbol{\mu}}_c^{(t + 1)} \right)}{\sum_i \lambda_{i,c}^{(t)}}
\end{equation}
The vectors are re-assigned to a cloud layer at the end of each parameters update, applying the maximum a posteriori (MAP) criterion
\begin{equation}
    \begin{split}
        \lambda_{i,2}^{(t + 1)} &= \underset{c}{\operatorname{argmax}} \ p \left( \tilde{\mathbf{v}}_i \mid {\boldsymbol{\mu}}_c^{(t + 1)}, {\boldsymbol{\Sigma}}_c^{(t + 1)} \right) - 1 \\
        \lambda_{i,1}^{(t + 1)} &= 1 - \lambda_{i,2}^{(t + 1)}.  
    \end{split}
\end{equation}
After completing the inference of the velocity vectors distribution, it is possible to infer the cloud layer's height using the same method. The velocity vectors in an image were calculated using the WLK method. The algorithm approximates the velocity vector using a set of pixels inside a window. The result is that the velocity vectors do not exactly correspond to a clouds' pixels, which are in motion. Instead, the velocity vectors are assigned to nearby pixels. To identify which layer of clouds $c$, is the highest and which one is the lowest, the height distribution of the pixels is inferred using the MAP classification of the velocity vectors $\mathbf{v}^\prime_{i,j}$ in a image. 

The height of the pixels within the cloud are modelled as independently distributed normal random variables $H_{i,j} \sim \mathcal{N} (\mu_c, \sigma^2_c) $. The probabilistic model to infer the distribution of heights of each cloud layer in a frame is,
\begin{equation}
	\label{eq:height_distributions}
    \log p \left( H_{i,j} \mid \boldsymbol{\Theta} \right) \propto \rho_{i,j,1} \cdot \log p \left( H_{i,j} \mid \mu_1, \sigma^2_1 \right) + \rho_{i,j,2} \cdot \log p \left( H_{i,j} \mid \mu_2, \sigma^2_2 \right),
\end{equation}
where $\boldsymbol{\Theta} = \{\boldsymbol{P}, \mu_1, \sigma_1, \mu_2, \sigma_2 \}$, and $\rho_{i,j,c} \in \{0, 1\}$ is a convex variable so that $\rho_{i,j,2} = 1 - \rho_{i,j,1}$.

The ICM algorithm is also used to the infer the parameters of the height distributions model. The $\rho_{i,j,c}$ are initialized to the MAP classification of the velocity vectors $\mathbf{v}^\prime_{i,j}$ using the parameters that were inferred using all the velocity vectors $\tilde{\mathbf{v}}_i$ in Eq. \eqref{eq:dataset},
\begin{equation}
    \begin{split}
        \rho_{i,j,2} &= \underset{c}{\operatorname{argmax}} \ p \left( \mathbf{v}^{\prime}_{i,j} \mid \boldsymbol{\mu}_c, \boldsymbol{\Sigma}_c \right) - 1\\
    \rho_{i,j,1} &= 1 - \rho_{i,j,2}.   
    \end{split}
\end{equation}
The parameters of the height distributions are updated using the formulas in Eq. \eqref{eq:parameters_estimation}. The algorithm eventually converges so that the pixels in the frame are segmented where a cloud appears. The segmentation is performed according to the MAP classification of height distributions,
\begin{equation}
    \begin{split}
        \rho_{i,j,2}^{(t + 1)} &= \underset{c}{\operatorname{argmax}} \ p \left( H_{i,j} \mid \mu_c^{(t + 1)}, \sigma_c^{2(t + 1)}\right) - 1\\
        \rho_{i,j,1}^{(t + 1)} &= 1 - \rho_{i,j,2}^{(t + 1)}. 
    \end{split}
\end{equation}
In order to find the height of a given cloud layer, the heights are averaged with this formula,
\begin{equation}
    \bar{H}_c = \frac{\sum_{i,j} \rho_{i,j,c} \cdot H_{i,j} \cdot \mathbb{I} \left( b_{i,j} = 1 \right)}{\sum_{i,j} \rho_{i,j,c} \cdot \mathbb{I} \left( b_{i,j} = 1 \right)}.
\end{equation}
The wind velocity fields are organized into upper and lower layers by average height $\bar{H}_c$. In this way, each detected wind velocity field has a distribution of velocity vectors, and another distribution of heights.

\subsubsection{Sampling}

In order to reduce the computational burden of the algorithm, a subset of the velocity vectors is selected according to the estimated probability distributions of the vectors. At each layer $c$, we define the importance weights $w_{i,c}^k$ as
\begin{equation}
    w^k_{i,c} \triangleq p \left( \tilde{\mathbf{v}}^k_i \middle| \boldsymbol{\theta}_c \right), \quad w_{i,c}^k \in \mathbb{R}^+.
\end{equation}
The weights are normalized to have the characteristics of a probability mass function such as $\sum_{i = 1}^{N_k} \hat w_{i,c}^k = 1$. 

The Cumulative Probability Function (CDF) is computed as
\begin{equation}
    \tilde{w}^k_{i,c} = \left\{ \sum_{m = 1}^i \hat{w}^k_{m,c} \right\}_{i = 1}^{N^k}.
\end{equation}
In order to select samples for each distribution $p ( \tilde{\mathbf{v}}^k_i \mid \boldsymbol{\theta}_c )$, $N^*/C$ samples are drawn from a uniform distribution,
\begin{equation}
    z_{j,c}^k \sim \mathcal{U}\left( 0, 1 \right), \quad j = 1, \ldots, \frac{N^*}{C},
\end{equation}
For each value $z_{j,c}^k$, a sample is selected with the criterion 
\begin{equation}
    I_{j,c}^k = \operatorname{argmin} \ \mid \tilde{w}_{i,c}^k - z_{j,c}^k \mid, \ \forall i = 1, \ldots, N_k \ \forall j = 1, \ldots, \frac{N^*}{C}.
\end{equation}
The selected vectors are the ones whose CDF is closest to the values of the uniform samples $z_{j,c}^k$,
\begin{equation}
    \tilde{\mathbf{v}}_c^{*k} \triangleq \tilde{\mathbf{v}}^k_{I_{j,c}^k}, \quad \forall j = 1, \ldots, \frac{N^*}{C}.
\end{equation}

The subset of selected velocity vectors in frame $k$ for the cloud layer $c$ is $\mathbf{V}_c^{*k} = \{ ( \tilde{u}, \tilde{v} )_{j,c}^{*k} \in \mathbb{R}^2 \mid \forall j = 1, \ldots, N^*/C \} $, the subset of Euclidean coordinate pairs of those selected vectors is $\mathbf{X}_c^{*k} = \{ ( x, y )_{j,c}^{*k} \in \mathbb{N}^2 \mid \forall j = 1, \ldots, N^*/C \}$. 

Assuming that the prior is uniform, the posterior probabilities are,
\begin{equation}
    \label{eq:posterior_proba}
    z_{i,c}^{*k} \triangleq \frac{p \left( \tilde{\mathbf{v}}^{*k}_i \middle| \boldsymbol{\theta}_c \right)}{\sum_{c = 1}^C p \left( \tilde{\mathbf{v}}^{*k}_i \middle| \boldsymbol{\theta}_c \right)}.
\end{equation}

The sampling is repeated for as many cloud layers detected. All selected subsets of vectors, coordinate pairs, and weights form the dataset that is used to approximate the wind velocity field, 
\begin{equation}
    \label{eq:selected_dataset}
    \mathbf{X}^{*k} = 
      \begin{bmatrix}
        x^{*k}_1 & y^{*k}_1 \\
        \vdots & \vdots  \\
        x^{*k}_{N^*} & y^{*k}_{N^*} \\
      \end{bmatrix}, \
    \mathbf{V}^{*k} = 
      \begin{bmatrix}
        \tilde{v}^{*k}_1 & \tilde{u}^{*k}_1 \\
        \vdots & \vdots  \\
        \tilde{v}^{*k}_{N^*} & \tilde{u}^{*k}_{N^*} \\
      \end{bmatrix}, \
    \mathbf{Z}^{*k} = 
      \begin{bmatrix}
        z^{*k}_{1,1} & z^{*k}_{1,c} \\
        \vdots & \vdots  \\
        z^{*k}_{N^*,1} & z^{*k}_{N^*,c} \\
      \end{bmatrix},
\end{equation}
where $N^k >> N^*$. 

\section{Flow Visualization}

The atmosphere is a system where the dynamics are continuously changing \cite{KALNAY2003}. This fact implies that a wind velocity field exists, but we can only visualize it where clouds are present. From ground level to the Tropopause, the wind flow can have multiple layers with different velocities in each one of the layers. The wind flow may also be convective, however, for the sake of simplicity, we assume that the multi-layer flow which is observed in IR images is a multi-layer laminar flow. This analysis neither considers the z-component in the motion of a cloud (which is not observable)  nor the possible inter-crossing of cloud layers.

\subsection{Wind Velocity Field Estimation}

Three methods were implemented to estimate the extrapolation function and compare their performances. The first method uses a weighted $\varepsilon$-support vector regression machine  ($\varepsilon$-WSVM) for each one of the velocity components. The second method is a $\varepsilon$-MO-WSVM that estimates both velocity components. The third is an innovation which uses a $\varepsilon$-MO-WSVM with flow constraints ($\varepsilon$-MO-WSVM-FC) to estimate both velocity components. The flow constraints are used to force the extrapolated wind flow to have zero divergence or curl, so it can be assumed that, in the approximated wind flow, streamlines are equivalent to the cloud pathlines.

The regression problem can be formulated as the optimization of a function with the form,
\begin{equation}
    f \left(\mathbf{x}_i\right) = \mathbf{w}^\top \varphi \left( \mathbf{x}_i \right) + b, \ \forall i = 1, \dots, N^*, \ \mathbf{w}, \mathbf{x}_i \in \mathbb{R}^D,\ b \in \mathbb{R}.
\end{equation}
where $\mathbf{x}_i \triangleq \mathbf{x}^{*k}_i$  in our problem, and where $\varphi(\cdot)$ is a transformation into a higher dimensional (possibly infinite) Hilbert space $\mathcal{H}$ endowed with a dot product $\mathcal{K}({\bf x}_i,{\bf x}_j)=\langle \varphi({\bf x}_i),\varphi({\bf x}_j)$. A function  $\mathcal{K}({\bf x}_i,{\bf x}_j)$ is a dot product if it is a bivariate positive semi-definite function that maps ${\bf x}_i,{\bf x}_j$ into $\mathbb{R}$, commonly called a Mercer's kernel or simply a kernel function. 

\subsubsection{Support Vector Machine for Regression}

Assuming $\mathbf{v}_i =\{u_i,v_i\} \triangleq \mathbf{v}_i^{*k}$, the regression problem in a $\varepsilon$-SVM is formulated with an $\varepsilon$-insensitive loss function, which penalizes the errors $ |\varepsilon| > 0$ \cite{DRUCKER1997} for each one of the components in ${\bf v}_i$ and for each cloud layer $c$ as
\begin{equation}
    \left| u_i - f \left( \mathbf{x}_i \right)\right|_{\varepsilon} = \max \left[ 0, \left| u_i - f \left( \mathbf{x}_i \right)\right|-\varepsilon \right], \ \forall i = 1, \dots, N, \ u_i,\varepsilon \in \mathbb{R},
\end{equation}
and identically for $v_i$. The $\varepsilon$-insensitive loss function can be seen as a tube of radius $\varepsilon$ adjusted around the regression hyper-plane via the Support Vectors (SV) \cite{SCHOLKOPF2000}.

The samples are weighted by their probability of belonging to wind velocity field $c$ \cite{ELATTAR2010},
\begin{equation}
    \begin{split}
        z_i &\triangleq z_i^{*k}, \quad z_i \in \mathbb{R}^{\leq 1}. \\
        c_i &= z_i \cdot \frac{C}{N}       
    \end{split}
\end{equation}
The L2-norm and $\varepsilon$-loss function is applied to the model weights, 
\begin{equation}
    \label{eq:primal}
    \begin{split}
    \min_{\mathbf{w}, b, \xi, \xi^*} & \quad \frac{1}{2} \| \mathbf{w} \|^2 + \frac{C}{N} \sum_{i = 1}^N z_i \left( \xi_i + \xi_i^* \right) \\ 
    \mathrm{s.t.} & 
    \begin{cases}
        u_{i}-\mathbf{w}^\top \varphi \left( \mathbf{x}_i \right) - b & \leq \varepsilon + \xi_i \\
        \mathbf{w}^\top \varphi \left( \mathbf{x}_i \right) + b  - u_{i} & \leq \varepsilon + \xi_i^* \\
        \xi_i, \xi_i^* & \geq 0
    \end{cases}  \quad i = 1, \ldots, N, 
    \end{split}
\end{equation}
and identically for $v_i$. The slack variables $\xi_i$ were introduced to relax the constraints of the optimization problem and to deal with unfeasible optimization problems \cite{CORTES1995}. The primal objective function aims to find the trade off between the regularization term $\varepsilon$, the allowed errors or slack variables $\xi_i$ and $\xi_i^*$, and the complexity of the model $c_i$ per weighted sample.

The proposed kernel functions in this analysis are, 
\begin{equation}
    \begin{split}
        \mathcal{K} \left( \mathbf{x}_i, \mathbf{x}_j \right) &= \mathbf{x}_i^\top \mathbf{x}_j, \\ 
        \mathcal{K} \left( \mathbf{x}_i, \mathbf{x}_j \right) &= \exp \left( - \gamma \cdot || \mathbf{x}_i - \mathbf{x}_j ||^2 \right), \\
        \mathcal{K} \left( \mathbf{x}_i, \mathbf{x}_j \right) &= \left( \gamma \cdot \mathbf{x}_i^\top \mathbf{x}_j + \beta \right)^d,        
    \end{split}
\end{equation}
where $\gamma, \ \beta \in \mathbb{R}$, and $d \in \mathbb{N}$ are the kernel hyperparameters that need cross-validation. \cite{SCHOLKOPF2000}. These kernel functions are referred to as linear, radial basis function (RBF) or square exponential, and polynomial of order $d$ respectively \cite{SHAWE2004}.

In order to optimize the constrained problem in functional \eqref{eq:primal} and constraints \eqref{eq:primal_constraints} a Langrangian functional is constructed with the functional and the set of constraints through a dual set of new variables \cite{SMOLA2004}, which leads to a solvable Quadratic Programming problem (QP). The Lagrangian functional is 
\begin{equation}
    \begin{split}
        \mathcal{L} & \left( \mathbf{w}, b,\alpha, \alpha^*, \beta, \xi, \xi^*, \varepsilon, \eta, \eta^* \right) = \\
        & = \frac{1}{2} \| \mathbf{w} \|^2 + c_i \sum_{i = 1}^N \left( \xi_i + \xi_i^* \right) \ \ldots \\
        & - \sum_{i = 1}^N \left( \eta_i \xi_i + \eta_i^* \xi_i* \right) - \sum_{i = 1}^N \alpha_i \left( \varepsilon + \xi_i - u_i + \mathbf{w}^\top \varphi \left( \mathbf{x}_i \right) + b \right) \ \ldots \\
        & - \sum_{i = 1}^N \alpha_i^* \left( \varepsilon + \xi_i^* + u_i -  \mathbf{w}^\top \varphi \left( \mathbf{x}_i \right)- b \right), \quad \forall i = 1, \dots, N, \quad \eta_i, \eta_i^* \in \mathbb{R}.  
    \end{split}
\end{equation}
The derivatives of the primal variables $\mathbf{w},\varepsilon, \xi_i, \xi_i^*$  yield to the following set of equations, which is a case of Karush-Kuhn-Tucker (KKT) conditions,
\begin{equation}
    \begin{split}
        \mathbf{w}^\top &= \sum_{i = 1}^N \left( \alpha_i^* - \alpha_i \right) \varphi \left( \mathbf{x}_i \right), \\
        0 &= \sum_{i = 1}^N \left( \alpha_i - \alpha_i^* \right ), \\
        0 &= c_i - \alpha_{i} - \eta_{i}, \\
        0 &= c_i 
        - \alpha_{i}^* - \eta_{i}^*.
    \end{split}
\end{equation}
These conditions, together with the complimentary KKT conditions (which force the product of dual parameters $\alpha_i,\alpha^*_i$ with the constraints to be zero) leads to the following dual functional by substitution on the Lagrangian: 
\begin{equation}
    \begin{split}
        \min_{\boldsymbol{\alpha}, \boldsymbol{\alpha}^*} &\quad \frac{1}{2} \cdot \left( \boldsymbol{\alpha} - \boldsymbol{\alpha}^* \right)^\top \mathbf{K} \left( \boldsymbol{\alpha} - \boldsymbol{\alpha}^* \right) + \sum_{i=1}^N \left( {\alpha_i} - \alpha_i^* \right)u_i + \varepsilon \cdot  \mathbf{1}^\top \left( \boldsymbol{\alpha} + \boldsymbol{\alpha}^* \right) \\
        &\mathrm{s.t.}
        \begin{cases} 
            \mathbf{1}^\top \left( \boldsymbol{\alpha} - \boldsymbol{\alpha}^* \right) = 0 \\ 
            0 \leq \alpha_i, \alpha_i^* \leq c_i
        \end{cases} \ \forall i = 1, \dots, N.   
    \end{split}
\end{equation}
where $\mathbf{1}_{1 \times N} = [1, \ldots, 1 ]^\top$, and matrix $\bf{K}$ is a Gram matrix of dot product such that ${\bf K}_{i,j} = \mathcal{K}({\bf x}_i,{\bf x}_j) $. The minimal of the primal function is equivalent to the saddle point on the Lagrangian formulation. The approximated function is,
\begin{equation}
    f \left( \mathbf{x} \right) = \sum_{i = 1}^N  \left(\alpha_i  - \alpha^*_{i}\right) \cdot \mathcal{K} \left( \mathbf{x}_i, \mathbf{x}_i \right) + b,
\end{equation}
where $b$ is obtained from the complimentary KKT conditions. 

\subsubsection{Multi-Ouput Weighted Support Vector Machine}

When the wind velocity field function is approximated by $\varepsilon$-MO-SVM,the primal regression can be formulated as 
\begin{equation}
    {\bf v}_i = {\bf W}^\top\varphi({\bf x}_i)+{\bf b},
\end{equation}
where each one of the column vectors of primal parameter matrix ${\bf W}$ approximates one of the velocities in vector ${\bf y}_i$. Primal parameters are a function of the dual parameters as well, but the dual parameters $\boldsymbol{\alpha}_i, \boldsymbol{\alpha}_i^{*}$ are vectors in a $2$-dimensional multi-output problem. 

Since independent variables are represented in vectors ${\bf v}_i$, the training set is defined in a vector  $\tilde{\mathbf{v}}_{1 \times 2N}$, and so are the dual parameters $\tilde{\boldsymbol{\alpha}}_{1 \times 2N}$ and $\tilde{\boldsymbol{\alpha}}^*_{1 \times 2N} $ for notation simplicity.

The gram matrix of dot products between input patterns $\varphi({\bf x}_i)$ can be interpreted as the covariance matrix between variables ${\bf v}_i$. Indeed
\begin{equation}
    \begin{split}
        \mathbb{E}\left(({\bf v}_i-{\bf b}^\top)({\bf v}_j-{\bf b})\right) &= \mathbb{E}\left(   {\bf W}^\top \varphi({\bf x}_i) \varphi({\bf x}_j)^\top{\bf W}\right) \\
        &= \left( \begin{array}{cc}
        \varphi({\bf x}_i)^\top \Sigma_{11} \varphi({\bf x}_j)&\varphi({\bf x}_i)^\top \Sigma_{12}\varphi({\bf x}_j)\\
        \varphi({\bf x}_i)^\top \Sigma_{21}\varphi({\bf x}_j)&\varphi({\bf x}_i)^\top \Sigma_{22}\varphi({\bf x}_j)\\
        \end{array} \right),
    \end{split}
\end{equation}
where the $2\times2$ covariance $ \mathbb{E}\left({\bf W}{\bf W}^\top\right) $ is interpreted as a model for the dependencies between elements in ${\bf v}_i$, i.e. 
\begin{equation}
    \mathbb{E}\left({\bf W}{\bf W}^\top\right)=
    \left(\begin{array}{cc}
    \Sigma_{11} & \Sigma_{12}\\
    \Sigma_{21} & \Sigma_{22}
    \end{array}\right).
\end{equation}

If we consider that both vertical and horizontal velocities are independent, then $\Sigma_{12}=\Sigma_{21}={\bf 0}$. If we assume further that $\Sigma_{11}=\Sigma_{22}={\bf I}$ for simplicity, which, in turn leads to
\begin{equation}
    \mathbb{E}\left(({\bf v}_i-{\bf b}^\top)({\bf v}_j-{\bf b})\right) =
    \left(\begin{array}{cc}
    \mathcal{K}({\bf x}_i,{\bf x}_j)&0\\
    0&\mathcal{K}({\bf x}_i,{\bf x}_j)\\
    \end{array}\right).
\end{equation}

The Gram matrix $\tilde{\mathbf{K}}_{DN \times DN}$ in the $\varepsilon$-MO-SVM formulation for independent components is,
\begin{equation}
    \tilde{\mathbf{K}} = \left( \begin{array}{cc}
        \mathbf{K} & \mathbf{0} \\ 
        \mathbf{0} & \mathbf{K}
    \end{array} \right).
\end{equation}
The full kernel matrix in a $\varepsilon$-MO-WSVM is computationally expensive, and it is not implemented in this research.

The extension of weights in the $\varepsilon$-MO-WSVM requires weighting each sample in each output \cite{HAN2014}, 
\begin{equation}
    \begin{split}
        \tilde{z}_i &= \left[ z \ldots z_N \ z_1 \ldots z_N \right]^\top, \quad
        \sum_{i = 1}^{D \cdot N} \tilde{z}_i = 2, \quad \tilde{z}_i \in \mathbb{R}^{\leq 1}.
    \end{split}
\end{equation}

The dual formulation of the QP problem for the $\varepsilon$-MO-WSVM is,
\begin{equation}
    \label{eq:dual_formaulation}
    \begin{split}
        \min_{\tilde{\boldsymbol{\alpha}}, \tilde{\boldsymbol{\alpha}}^*} & \quad \frac{1}{2} \cdot \left( \tilde{\boldsymbol{\alpha}} - \tilde{\boldsymbol{\alpha}}^* \right)^\top \tilde{\mathbf{K}} \left( \tilde{\boldsymbol{\alpha}} - \tilde{\boldsymbol{\alpha}}^* \right) + \tilde{\mathbf{y}}^\top \left( \tilde{\boldsymbol{\alpha}} - \tilde{\boldsymbol{\alpha}}^* \right) + \varepsilon \cdot \mathbf{1}^\top \left( \tilde{\boldsymbol{\alpha}} + \tilde{\boldsymbol{\alpha}}^* \right) \\
        &\mathrm{s.t.}
        \begin{cases} 
            \mathbf{1}^\top \left( \tilde{\boldsymbol{\alpha}} - \tilde{\boldsymbol{\alpha}}^* \right) = 0 \\ 
            \mathbf{0} \leq \tilde{\alpha}_i, \tilde{\alpha}_i^* \leq \tilde{c}_i \\
        \end{cases}  \ \forall i = 1, \dots, 2 N,  
    \end{split}
\end{equation}
where the extended weighted complexity is $\tilde{c_i} = \tilde{z}_i / 2N$.

\subsubsection{Multi-Ouput Weighted Support Vector Machine with Flow Constraints}

Assuming that the analyzed air parcel is sufficiently small so that the flow can be considered approximately incompressible and irrotational, a new set of flow constraints are added to the original set of constraints with the purpose of visualizing the wind velocity field to force the divergence and the vorticity to zero:
\begin{equation}
    \label{eq:flow_constraints}
    \mathrm{s.t.}
    \begin{cases} 
        \left( \tilde{\mathbf{v}}^{k\top}_c \mathbf{\Delta}_{x,y} \mathbf{\dot{V}} \right)  \cdot \left( \tilde{\mathbf{v}}^{k\top}_c \mathbf{\Delta}_{x,y} \mathbf{\dot{V}} \right)^\top &= 0 \\
        \left(  \tilde{\mathbf{v}}^{k\top}_c \mathbf{\Delta}_{x,y} \mathbf{\dot{D}} \right) \cdot \left( \tilde{\mathbf{v}}^{k\top}_c \mathbf{\Delta}_{x,y} \mathbf{\dot{D}} \right)^\top &= 0,
    \end{cases} 
\end{equation}
where the matrices of this expression are defined in Eq. \eqref{eq:matrix_1} Eq. \eqref{eq:set_matrix_1} and Eq. \eqref{eq:set_matrix_2}. To compute the vorticity and divergence, the differentiation of the velocity field along the x-axis, the and y-axis is implemented using operator
\begin{equation}
    \label{eq:matrix_1}
    \mathbf{\Delta}_{x,y} =
    \begin{bmatrix}
        \boldsymbol{\Delta}_x & \mathbf{0} \\
        \mathbf{0} & \boldsymbol{\Delta}_y
    \end{bmatrix}_{2N \times 2N},
\end{equation}
where the differential operators $\boldsymbol{\Delta}_x$ and $\boldsymbol{\Delta}_y$ are defined as,
\begin{equation}
    \label{eq:set_matrix_1}
    \boldsymbol{\Delta}_x =
    \begin{bmatrix}
        -1 & 0 & \ldots & 0\\
        1 & -1 & \ddots & \vdots \\
        0 & 1 & \ddots & 0 \\
        \vdots &  \ddots & \ddots & -1\\
        0 & \ldots & 0 & 1
    \end{bmatrix}_{N \times N}; \quad
    \boldsymbol{\Delta}_y =
    \begin{bmatrix}
        -1 & \ldots & 0 \\
        \vdots & \ddots  & \vdots  \\
        0 & \ldots & -1 \\
        1 & \ldots & 0  \\
        \vdots & \ddots & \vdots \\
        0 & \ldots & 1
    \end{bmatrix}_{N \times N}.
\end{equation}
The operators of the velocity field's vorticity and divergence are respectively,
\begin{equation}
    \label{eq:set_matrix_2}
    \mathbf{\dot{V}} = \left[ \mathbf{I} \quad \mathbf{I} \right]^\top_{2N \times N}, 
    \mathbf{\dot{D}} = \left[ \mathbf{I} \quad -\mathbf{I} \right]^\top_{2N \times N}
\end{equation}

The velocity field is extrapolated to the entire frame using the inferred parameters in frame $k$
\begin{equation}
    \label{eq:extrapolation}
    \hat{\mathbf{v}}^k_c = \left( \tilde{\boldsymbol\alpha}^k_c - \tilde{\boldsymbol\alpha}^{*k}_c \right) \cdot \mathcal{K} \left( \mathbf{X}^{*k}, \mathbf{X} \right) + \mathbf{b}_c^k,
\end{equation}
where the velocity components are $\hat{\mathbf{U}}^k_c \triangleq \hat{\mathbf{v}}^k_{x,c}$, and $\hat{\mathbf{V}}^k_c \triangleq \hat{\mathbf{v}}^k_{y,c}$, where  $\hat{\mathbf{U}}_c^k, \hat{\mathbf{V}}^k_c \in \mathbb{R}^{M \times N} $. 

To compute the flow constraints, the velocity field has to be extrapolated to the whole frame using Eq. \eqref{eq:extrapolation}. The constraints in Eq. \eqref{eq:flow_constraints} are added to the constraints in the dual formulation of the $\varepsilon$-MO-SVM in Eq. \eqref{eq:dual_formaulation}. 


\section{Wind Velocity Field Streamlines}

To estimate the wind velocity field dynamics, velocity vectors are approximated using the WLK method. The velocity vectors are weighted by the posterior probabilities of the cloud layers in the image, and transformed to the cloud layer plane. The velocity vectors are segmented and sampled to reduce the noise and the computation burden. The parameters of the $\varepsilon$-MO-WSVM-FC are cross-validated, and the model is trained to estimate the wind velocity field of the detected cloud layers. If an optimal set of parameters is available, it is possible to proceed with the training of $\varepsilon$-MO-WSVM-FM without performing the cross-validation. After training the $\varepsilon$-MO-WSVM-FC, the testing is performed to extrapolate the wind velocity field to the whole image. The streamlines are computed using Eq. \eqref{eq:streamlines} to visualize the trajectory of a cloud. The potential lines are not shown in the Fig. \ref{fig:day_2_layer_0_turbulent}-\ref{fig:day_5_layer_1}, but they are computed with Eq. \eqref{eq:potential_lines}.

The physical process of cloud formation and evolution over time is part of atmospheric thermodynamics and may have divergence and vorticity \cite{LAMB2011}. The air parcel in one frame is very small compared to the whole volume of air contained in the atmosphere. Within this frame we consider it feasible that there is no vorticity or divergence, and the approximated streamlines are equivalent to the pathlines. Henceforth, the obtained results are a numerical approximation of the actual atmospheric air parcel flow.

When we assume that a flow does not have divergence and vorticity, the stream and velocity potential functions are orthogonal, and we can apply Cauchy-Riemann equations to calculate their rates of change \cite{GRANGER1995}. For the stream function we determine $d \phi = v_x dy - v_y dx$ using samples of functions. The trapezoidal rule of numerical analysis is applied to solve the definite integrals \cite{DRAGOMIR1999}. The values of a streamline are,
\begin{equation}
    \label{eq:streamlines}
    \begin{split}
        \boldsymbol{\Phi}_c &= \frac{\hat{H}_c}{2}  \left\{ \sum^i_{m = 1} \hat{\bf u}_{m,c} \odot \Delta {\bf y}_{m,c} \right\}^N_{i = 1} \\
        &- \frac{\hat{H}_c}{2}\left\{ \sum^j_{m = 1} \hat{\bf v}_{m,c} \odot \Delta {\bf x}_{m,c} \right\}^N_{j = 1} ,
    \end{split}
\end{equation}
where $\odot$ denotes the element-wise matrix multiplication. This is the sum of element-wise products between each velocity component and its opposite differential increments.

%The total change in the potential function is $d\psi = v_x dx + v_y dy$, so we can determine the potential in each pixel $\mathbf{x} = \{x, y\}$ as,
%\begin{equation}
%    \boldsymbol{\Psi}_c = \frac{\hat{H}_c}{2} \left[ \left\{ \sum^j_{m = 1} \hat{\bf u}_{m,c} \odot \Delta {\bf x}_{m,c} \right\}^N_{j = 1} + \left\{ \sum^i_{m = 1} \hat{\bf v}_{m,c} \odot \Delta {\bf y}_{m,c}  \right\}^M_{i = 1}  \right].
%\end{equation}
%the sum of each element-wise product between the velocity components, and their differential increment. 

==> Wind%20Flow%20Estimation%20in%20Thermal%20Sky%20Images%20for%20Sun%20Occlusion%20Prediction%20(IEEE-PES-ISGT2021)-2/summary_methods.tex <==
\subsection{Wind Velocity Field Estimation}

Three methods were implemented to estimate the extrapolation function and compare their performances. The first method uses a weighted $\varepsilon$-support vector regression machine  ($\varepsilon$-WSVM) for each one of the velocity components. The second method is a $\varepsilon$-MO-WSVM that estimates both velocity components. The third is an innovation which uses a $\varepsilon$-MO-WSVM with flow constraints ($\varepsilon$-MO-WSVM-FC) to estimate both velocity components. The flow constraints are used to force the extrapolated wind flow to have zero divergence or curl, so it can be assumed that, in the approximated wind flow, streamlines are equivalent to the cloud pathlines.

The regression problem can be formulated as the optimization of a function with the form,
\begin{equation}
    f \left(\mathbf{x}_i\right) = \mathbf{w}^\top \varphi \left( \mathbf{x}_i \right) + b, \ \forall i = 1, \dots, N^*, \ \mathbf{w}, \mathbf{x}_i \in \mathbb{R}^D,\ b \in \mathbb{R}.
\end{equation}
where $\mathbf{x}_i \triangleq \mathbf{x}^{*k}_i$  in our problem, and where $\varphi(\cdot)$ is a transformation into a higher dimensional (possibly infinite) Hilbert space $\mathcal{H}$ endowed with a dot product $\mathcal{K}({\bf x}_i,{\bf x}_j)=\langle \varphi({\bf x}_i),\varphi({\bf x}_j)$. A function  $\mathcal{K}({\bf x}_i,{\bf x}_j)$ is a dot product if it is a bivariate positive semi-definite function that maps ${\bf x}_i,{\bf x}_j$ into $\mathbb{R}$, commonly called a Mercer's kernel or simply a kernel function. 

\subsubsection{Support Vector Machine for Regression}

Assuming $\mathbf{v}_i =\{u_i,v_i\} \triangleq \mathbf{v}_i^{*k}$, the regression problem in a $\varepsilon$-SVM is formulated with an $\varepsilon$-insensitive loss function, which penalizes the errors $ |\varepsilon| > 0$ \cite{DRUCKER1997} for each one of the components in ${\bf v}_i$ and for each cloud layer $c$ as
\begin{equation}
    \left| u_i - f \left( \mathbf{x}_i \right)\right|_{\varepsilon} = \max \left[ 0, \left| u_i - f \left( \mathbf{x}_i \right)\right|-\varepsilon \right], \ \forall i = 1, \dots, N, \ u_i,\varepsilon \in \mathbb{R},
\end{equation}
and identically for $v_i$. The $\varepsilon$-insensitive loss function can be seen as a tube of radius $\varepsilon$ adjusted around the regression hyper-plane via the Support Vectors (SV) \cite{SCHOLKOPF2000}.

The samples are weighted by their probability of belonging to wind velocity field $c$ \cite{ELATTAR2010},
\begin{equation}
    \begin{split}
        z_i &\triangleq z_i^{*k}, \quad z_i \in \mathbb{R}^{\leq 1}. \\
        c_i &= z_i \cdot \frac{C}{N}       
    \end{split}
\end{equation}
The L2-norm and $\varepsilon$-loss function is applied to the model weights, 
\begin{equation}
    \label{eq:primal}
    \begin{split}
    \min_{\mathbf{w}, b, \xi, \xi^*} & \quad \frac{1}{2} \| \mathbf{w} \|^2 + \frac{C}{N} \sum_{i = 1}^N z_i \left( \xi_i + \xi_i^* \right) \\ 
    \mathrm{s.t.} & 
    \begin{cases}
        u_{i}-\mathbf{w}^\top \varphi \left( \mathbf{x}_i \right) - b & \leq \varepsilon + \xi_i \\
        \mathbf{w}^\top \varphi \left( \mathbf{x}_i \right) + b  - u_{i} & \leq \varepsilon + \xi_i^* \\
        \xi_i, \xi_i^* & \geq 0
    \end{cases}  \quad i = 1, \ldots, N, 
    \end{split}
\end{equation}
and identically for $v_i$. The slack variables $\xi_i$ were introduced to relax the constraints of the optimization problem and to deal with unfeasible optimization problems \cite{CORTES1995}. The primal objective function aims to find the trade off between the regularization term $\varepsilon$, the allowed errors or slack variables $\xi_i$ and $\xi_i^*$, and the complexity of the model $c_i$ per weighted sample.

The proposed kernel functions in this analysis are, 
\begin{equation}
    \begin{split}
        \mathcal{K} \left( \mathbf{x}_i, \mathbf{x}_j \right) &= \mathbf{x}_i^\top \mathbf{x}_j, \\ 
        \mathcal{K} \left( \mathbf{x}_i, \mathbf{x}_j \right) &= \exp \left( - \gamma \cdot || \mathbf{x}_i - \mathbf{x}_j ||^2 \right), \\
        \mathcal{K} \left( \mathbf{x}_i, \mathbf{x}_j \right) &= \left( \gamma \cdot \mathbf{x}_i^\top \mathbf{x}_j + \beta \right)^d,        
    \end{split}
\end{equation}
where $\gamma, \ \beta \in \mathbb{R}$, and $d \in \mathbb{N}$ are the kernel hyperparameters that need cross-validation. \cite{SCHOLKOPF2000}. These kernel functions are referred to as linear, radial basis function (RBF) or square exponential, and polynomial of order $d$ respectively \cite{SHAWE2004}.

In order to optimize the constrained problem in functional \eqref{eq:primal} and constraints \eqref{eq:primal_constraints} a Langrangian functional is constructed with the functional and the set of constraints through a dual set of new variables \cite{SMOLA2004}, which leads to a solvable Quadratic Programming problem (QP). The Lagrangian functional is 
\begin{equation}
    \begin{split}
        \mathcal{L} & \left( \mathbf{w}, b,\alpha, \alpha^*, \beta, \xi, \xi^*, \varepsilon, \eta, \eta^* \right) = \\
        & = \frac{1}{2} \| \mathbf{w} \|^2 + c_i \sum_{i = 1}^N \left( \xi_i + \xi_i^* \right) \ \ldots \\
        & - \sum_{i = 1}^N \left( \eta_i \xi_i + \eta_i^* \xi_i* \right) - \sum_{i = 1}^N \alpha_i \left( \varepsilon + \xi_i - u_i + \mathbf{w}^\top \varphi \left( \mathbf{x}_i \right) + b \right) \ \ldots \\
        & - \sum_{i = 1}^N \alpha_i^* \left( \varepsilon + \xi_i^* + u_i -  \mathbf{w}^\top \varphi \left( \mathbf{x}_i \right)- b \right), \quad \forall i = 1, \dots, N, \quad \eta_i, \eta_i^* \in \mathbb{R}.  
    \end{split}
\end{equation}
The derivatives of the primal variables $\mathbf{w},\varepsilon, \xi_i, \xi_i^*$  yield to the following set of equations, which is a case of Karush-Kuhn-Tucker (KKT) conditions,
\begin{equation}
    \begin{split}
        \mathbf{w}^\top &= \sum_{i = 1}^N \left( \alpha_i^* - \alpha_i \right) \varphi \left( \mathbf{x}_i \right), \\
        0 &= \sum_{i = 1}^N \left( \alpha_i - \alpha_i^* \right ), \\
        0 &= c_i - \alpha_{i} - \eta_{i}, \\
        0 &= c_i 
        - \alpha_{i}^* - \eta_{i}^*.
    \end{split}
\end{equation}
These conditions, together with the complimentary KKT conditions (which force the product of dual parameters $\alpha_i,\alpha^*_i$ with the constraints to be zero) leads to the following dual functional by substitution on the Lagrangian: 
\begin{equation}
    \begin{split}
        \min_{\boldsymbol{\alpha}, \boldsymbol{\alpha}^*} &\quad \frac{1}{2} \cdot \left( \boldsymbol{\alpha} - \boldsymbol{\alpha}^* \right)^\top \mathbf{K} \left( \boldsymbol{\alpha} - \boldsymbol{\alpha}^* \right) + \sum_{i=1}^N \left( {\alpha_i} - \alpha_i^* \right)u_i + \varepsilon \cdot  \mathbf{1}^\top \left( \boldsymbol{\alpha} + \boldsymbol{\alpha}^* \right) \\
        &\mathrm{s.t.}
        \begin{cases} 
            \mathbf{1}^\top \left( \boldsymbol{\alpha} - \boldsymbol{\alpha}^* \right) = 0 \\ 
            0 \leq \alpha_i, \alpha_i^* \leq c_i
        \end{cases} \ \forall i = 1, \dots, N.   
    \end{split}
\end{equation}
where $\mathbf{1}_{1 \times N} = [1, \ldots, 1 ]^\top$, and matrix $\bf{K}$ is a Gram matrix of dot product such that ${\bf K}_{i,j} = \mathcal{K}({\bf x}_i,{\bf x}_j) $. The minimal of the primal function is equivalent to the saddle point on the Lagrangian formulation. The approximated function is,
\begin{equation}
    f \left( \mathbf{x} \right) = \sum_{i = 1}^N  \left(\alpha_i  - \alpha^*_{i}\right) \cdot \mathcal{K} \left( \mathbf{x}_i, \mathbf{x}_i \right) + b,
\end{equation}
where $b$ is obtained from the complimentary KKT conditions. 

\subsubsection{Multi-Ouput Weighted Support Vector Machine}

When the wind velocity field function is approximated by $\varepsilon$-MO-SVM,the primal regression can be formulated as 
\begin{equation}
    {\bf v}_i = {\bf W}^\top\varphi({\bf x}_i)+{\bf b},
\end{equation}
where each one of the column vectors of primal parameter matrix ${\bf W}$ approximates one of the velocities in vector ${\bf y}_i$. Primal parameters are a function of the dual parameters as well, but the dual parameters $\boldsymbol{\alpha}_i, \boldsymbol{\alpha}_i^{*}$ are vectors in a $2$-dimensional multi-output problem. 

Since independent variables are represented in vectors ${\bf v}_i$, the training set is defined in a vector  $\tilde{\mathbf{v}}_{1 \times 2N}$, and so are the dual parameters $\tilde{\boldsymbol{\alpha}}_{1 \times 2N}$ and $\tilde{\boldsymbol{\alpha}}^*_{1 \times 2N} $ for notation simplicity.

The gram matrix of dot products between input patterns $\varphi({\bf x}_i)$ can be interpreted as the covariance matrix between variables ${\bf v}_i$. Indeed
\begin{equation}
    \begin{split}
        \mathbb{E}\left(({\bf v}_i-{\bf b}^\top)({\bf v}_j-{\bf b})\right) &= \mathbb{E}\left(   {\bf W}^\top \varphi({\bf x}_i) \varphi({\bf x}_j)^\top{\bf W}\right) \\
        &= \left( \begin{array}{cc}
        \varphi({\bf x}_i)^\top \Sigma_{11} \varphi({\bf x}_j)&\varphi({\bf x}_i)^\top \Sigma_{12}\varphi({\bf x}_j)\\
        \varphi({\bf x}_i)^\top \Sigma_{21}\varphi({\bf x}_j)&\varphi({\bf x}_i)^\top \Sigma_{22}\varphi({\bf x}_j)\\
        \end{array} \right),
    \end{split}
\end{equation}
where the $2\times2$ covariance $ \mathbb{E}\left({\bf W}{\bf W}^\top\right) $ is interpreted as a model for the dependencies between elements in ${\bf v}_i$, i.e. 
\begin{equation}
    \mathbb{E}\left({\bf W}{\bf W}^\top\right)=
    \left(\begin{array}{cc}
    \Sigma_{11} & \Sigma_{12}\\
    \Sigma_{21} & \Sigma_{22}
    \end{array}\right).
\end{equation}

If we consider that both vertical and horizontal velocities are independent, then $\Sigma_{12}=\Sigma_{21}={\bf 0}$. If we assume further that $\Sigma_{11}=\Sigma_{22}={\bf I}$ for simplicity, which, in turn leads to
\begin{equation}
    \mathbb{E}\left(({\bf v}_i-{\bf b}^\top)({\bf v}_j-{\bf b})\right) =
    \left(\begin{array}{cc}
    \mathcal{K}({\bf x}_i,{\bf x}_j)&0\\
    0&\mathcal{K}({\bf x}_i,{\bf x}_j)\\
    \end{array}\right).
\end{equation}

The Gram matrix $\tilde{\mathbf{K}}_{DN \times DN}$ in the $\varepsilon$-MO-SVM formulation for independent components is,
\begin{equation}
    \tilde{\mathbf{K}} = \left( \begin{array}{cc}
        \mathbf{K} & \mathbf{0} \\ 
        \mathbf{0} & \mathbf{K}
    \end{array} \right).
\end{equation}
The full kernel matrix in a $\varepsilon$-MO-WSVM is computationally expensive, and it is not implemented in this research.

The extension of weights in the $\varepsilon$-MO-WSVM requires weighting each sample in each output \cite{HAN2014}, 
\begin{equation}
    \begin{split}
        \tilde{z}_i &= \left[ z \ldots z_N \ z_1 \ldots z_N \right]^\top, \quad
        \sum_{i = 1}^{D \cdot N} \tilde{z}_i = 2, \quad \tilde{z}_i \in \mathbb{R}^{\leq 1}.
    \end{split}
\end{equation}

The dual formulation of the QP problem for the $\varepsilon$-MO-WSVM is,
\begin{equation}
    \label{eq:dual_formaulation}
    \begin{split}
        \min_{\tilde{\boldsymbol{\alpha}}, \tilde{\boldsymbol{\alpha}}^*} & \frac{1}{2} \left( \tilde{\boldsymbol{\alpha}} - \tilde{\boldsymbol{\alpha}}^* \right)^\top \tilde{\mathbf{K}} \left( \tilde{\boldsymbol{\alpha}} - \tilde{\boldsymbol{\alpha}}^* \right) + \tilde{\mathbf{y}}^\top \left( \tilde{\boldsymbol{\alpha}} - \tilde{\boldsymbol{\alpha}}^* \right) + \varepsilon \mathbf{1}^\top \left( \tilde{\boldsymbol{\alpha}} + \tilde{\boldsymbol{\alpha}}^* \right) \\
        &\mathrm{s.t.}
        \begin{cases} 
            \mathbf{1}^\top \left( \tilde{\boldsymbol{\alpha}} - \tilde{\boldsymbol{\alpha}}^* \right) = 0 \\ 
            \mathbf{0} \leq \tilde{\alpha}_i, \tilde{\alpha}_i^* \leq \tilde{c}_i \\
        \end{cases}  \ \forall i = 1, \dots, 2 N,  
    \end{split}
\end{equation}
where the extended weighted complexity is $\tilde{c_i} = \tilde{z}_i / 2N$.

\subsubsection{Multi-Ouput Weighted Support Vector Machine with Flow Constraints}

Assuming that the analyzed air parcel is sufficiently small so that the flow can be considered approximately incompressible and irrotational, a new set of flow constraints are added to the original set of constraints with the purpose of visualizing the wind velocity field to force the divergence and the vorticity to zero:
\begin{equation}
    \label{eq:flow_constraints}
    \mathrm{s.t.}
    \begin{cases} 
        \left( \tilde{\mathbf{v}}^{k\top}_c \mathbf{\Delta}_{x,y} \mathbf{\dot{V}} \right)  \cdot \left( \tilde{\mathbf{v}}^{k\top}_c \mathbf{\Delta}_{x,y} \mathbf{\dot{V}} \right)^\top &= 0 \\
        \left(  \tilde{\mathbf{v}}^{k\top}_c \mathbf{\Delta}_{x,y} \mathbf{\dot{D}} \right) \cdot \left( \tilde{\mathbf{v}}^{k\top}_c \mathbf{\Delta}_{x,y} \mathbf{\dot{D}} \right)^\top &= 0,
    \end{cases} 
\end{equation}
where the matrices of this expression are defined in Eq. \eqref{eq:matrix_1} Eq. \eqref{eq:set_matrix_1} and Eq. \eqref{eq:set_matrix_2}. To compute the vorticity and divergence, the differentiation of the velocity field along the x-axis, the and y-axis is implemented using operator
\begin{equation}
    \label{eq:matrix_1}
    \mathbf{\Delta}_{x,y} =
    \begin{bmatrix}
        \boldsymbol{\Delta}_x & \mathbf{0} \\
        \mathbf{0} & \boldsymbol{\Delta}_y
    \end{bmatrix}_{2N \times 2N},
\end{equation}
where the differential operators $\boldsymbol{\Delta}_x$ and $\boldsymbol{\Delta}_y$ are defined as,
\begin{equation}
    \label{eq:set_matrix_1}
    \boldsymbol{\Delta}_x =
    \begin{bmatrix}
        -1 & 0 & \ldots & 0\\
        1 & -1 & \ddots & \vdots \\
        0 & 1 & \ddots & 0 \\
        \vdots &  \ddots & \ddots & -1\\
        0 & \ldots & 0 & 1
    \end{bmatrix}_{N \times N}; \quad
    \boldsymbol{\Delta}_y =
    \begin{bmatrix}
        -1 & \ldots & 0 \\
        \vdots & \ddots  & \vdots  \\
        0 & \ldots & -1 \\
        1 & \ldots & 0  \\
        \vdots & \ddots & \vdots \\
        0 & \ldots & 1
    \end{bmatrix}_{N \times N}.
\end{equation}
The operators of the velocity field's vorticity and divergence are respectively,
\begin{equation}
    \label{eq:set_matrix_2}
    \mathbf{\dot{V}} = \left[ \mathbf{I} \quad \mathbf{I} \right]^\top_{2N \times N}, 
    \mathbf{\dot{D}} = \left[ \mathbf{I} \quad -\mathbf{I} \right]^\top_{2N \times N}
\end{equation}

The velocity field is extrapolated to the entire frame using the inferred parameters in frame $k$
\begin{equation}
    \label{eq:extrapolation}
    \hat{\mathbf{v}}^k_c = \left( \tilde{\boldsymbol\alpha}^k_c - \tilde{\boldsymbol\alpha}^{*k}_c \right) \cdot \mathcal{K} \left( \mathbf{X}^{*k}, \mathbf{X} \right) + \mathbf{b}_c^k,
\end{equation}
where the velocity components are $\hat{\mathbf{U}}^k_c \triangleq \hat{\mathbf{v}}^k_{x,c}$, and $\hat{\mathbf{V}}^k_c \triangleq \hat{\mathbf{v}}^k_{y,c}$, where  $\hat{\mathbf{U}}_c^k, \hat{\mathbf{V}}^k_c \in \mathbb{R}^{M \times N} $. 

To compute the flow constraints, the velocity field has to be extrapolated to the whole frame using Eq. \eqref{eq:extrapolation}. The constraints in Eq. \eqref{eq:flow_constraints} are added to the constraints in the dual formulation of the $\varepsilon$-MO-SVM in Eq. \eqref{eq:dual_formaulation}. 

==> Wind%20Flow%20Estimation%20in%20Thermal%20Sky%20Images%20for%20Sun%20Occlusion%20Prediction%20(IEEE-PES-ISGT2021)-2/table_arxiv.tex <==
\begin{table}
    \centering
    \small
    \setlength{\tabcolsep}{3.5pt}
    \renewcommand{\arraystretch}{1.5}
        \begin{tabular}{lccccccccccccc}
        \toprule
        {} & \multicolumn{4}{c}{Parameters} & \multicolumn{4}{c}{Cross-Validated} & \multicolumn{5}{c}{Fixed} \\
        $\mathcal{K} \left(\mathbf{x}, \mathbf{x}^*\right) $ & $C$ & $\varepsilon$ & $\gamma$ & $\beta$ & MAE & WMAE & $\nabla \cdot \vec{V}$ & $\nabla \times \vec{V}$ & MAE & WMAE & $\nabla \cdot \vec{V}$ & $\nabla \times \vec{V}$ & Time [s] \\
        \midrule
        {} &  \multicolumn{13}{c}{$\varepsilon$-MO-WSVM} \\
        \midrule
        Linear & 31.06 & 0.31 & & & 13.27 & \textbf{12.49} & \textbf{1.30}$\mathbf{\cdot 10^3}$ & \textbf{1.35}$\mathbf{\cdot 10^3}$ & 13.17 & \textbf{12.45} & \textbf{1052.43} & \textbf{1196.68} & 19.95 \\
        RBF & 38.71 & 0.36 & 17.81 & & 14.00 & 13.13 & 1.21$\cdot 10^3$ & 1.22$\cdot 10^3$ & 13.83 & 12.87 & 620.99 & 641.04 & 12.22 \\
        $\mathcal{P}^2$ & 34.73 & 0.28 & 4.65 & 10.66 & 14.25 & 13.53 & 1.43$\cdot 10^4$ & 1.71$\cdot 10^4$ & 17.69 & 16.89 & 5.45$\cdot 10^4$ & 6.54$\cdot 10^4$ & 32.49 \\
        $\mathcal{P}^3$ & 38.47 & 0.22 & 4.19 & 2.33 & 19.29 & 18.12 & 8.89$\cdot 10^5$ & 8.93$\cdot 10^5$ & 42.77 & 43.03 & 1.84$\cdot 10^6$ & 2.16$\cdot 10^6$ & 44.77 \\
        \midrule
        {} & \multicolumn{13}{c}{$\varepsilon$-MO-WSVM-FC} \\
        \midrule
        Linear & 38.50 & 0.19 & & & 13.47 & \textbf{13.31} & \textbf{0} & \textbf{0} & 13.57 & 13.32 & 0 & 0.01 & 55.53 \\
        RBF & 38.52 & 0.35 & 13.92 & & 14.09 & 13.72 & 24.48 & 24.25 & 13.65 & \textbf{13.31} & \textbf{131.74} & \textbf{132.01} & \textbf{109.82} \\
        $\mathcal{P}^2$ & 39.72 & 0.24 & 3.78 & 44.8 & 14.37 & 13.96 & 61.06 & 98.00 & 15.10 & 14.75 & 477.77 & 367.05 & 125.79 \\
        $\mathcal{P}^3$ & 12.88 & 0.22 & 5.61 & 8.34 & 61.65 & 63.62 & 3.30$\cdot 10^7$ & 3.53$\cdot 10^7$ & 51.43 & 50.40 & 2.22$\cdot 10^6$ & 2.19$\cdot 10^6$ & 139.99 \\
        \bottomrule
    \end{tabular}
    \caption{The table shows the results obtained approximating the wind flow in the testing sequences when the parameters were cross-validated and when they were fixed to the optimal.}
    \label{tab:wsvm_fc}
\end{table}

==> methods.tex <==
\section{Multiple Wind Velocity Field Estimation}

\subsection{Velocity Vectors Calculation}

\subsubsection{Beta Mixture Model}

Consider the temperatures $\bar{T}_{i,j}$ of a given image (by omitting superindex $k$). The distribution of the normalized temperatures can be approximated by a mixture of beta distributions $\bar{T} \sim Be ( \alpha_c, \beta_c )$ with the density function,
\begin{equation}
    \label{eq:beta_distribution}
    f \left( \bar{T}_{i,j} ; \alpha_c, \beta_c \right) = \frac{1}{\mathrm{B} \left( \alpha_c, \beta_c \right)} \cdot \bar{T}_{i,j}^{\alpha_c - 1} \cdot \left( 1 - \bar{T}_{i,j}\right)^{\beta_c - 1}, \quad \alpha_c, \beta_c > 0,
\end{equation}
where $\bar{T}_{i,j} \in (0, 1)$,  the beta function is $\mathrm{B} ( \alpha_c, \beta_c ) = [ \Gamma ( \alpha_c ) \Gamma ( \beta_c ) ] / [\Gamma ( \alpha_c + \beta_c ) ] $, and the gamma function is $\Gamma ( \alpha_c ) = ( \alpha_c - 1 ) !$.

The log-likelihood of the beta density function that we need to compute the expected complete data log-likelihood (CDLL) is,
\begin{equation}
    \log p \left( \bar{T}_{i,j}\mid \alpha_c, \beta_c \right) = \left( \alpha_c - 1 \right) \log \bar{T}_{i,j}+ \left( \beta_c - 1 \right) \log \left( 1 - \bar{T}_{i,j} \right)- \log \mathrm{B} \left(\alpha_c, \beta_c \right),
\end{equation}
and the CDLL in a mixture model is,
\begin{equation}\label{EM_likelihood}
   \mathcal{Q} \left( \boldsymbol{\theta}^{\left( t\right)}, \boldsymbol{\theta}^{\left(t - 1\right)}\right) = \sum_{i = 1}^M \sum_{j = 1}^N \sum_{c = 1}^C \gamma_{i,j,c} \log \pi_c + \sum_{i = 1}^M \sum_{j = 1}^N \sum_{c = 1}^C \gamma_{i,j,c}  \log p \left( \bar{T}_{i,j} \mid \boldsymbol{\theta}^{\left( t\right)} \right)
\end{equation}
where $\gamma_{i,j,c} \triangleq  p ( y_{i,j} = c \mid \bar{T}_{i,j}, \boldsymbol{\theta}^{(t - 1)} )$ is the responsibility of the cluster $c$ in the sample $i,j$ and $\boldsymbol{\theta}^{( t)} = \{\alpha_c^{\left( t\right)} , \beta_c^{( t)} \}$.

The parameters in the clustering of beta distributions can be directly computed applying the Expectation Maximization (EM) algorithm \cite{MURPHY2012}. In the E stage of the algorithm a prior is established and then, by using the likelihood function \eqref{EM_likelihood}, a posterior $\gamma_{i,j,c} = p(y_{i,j} = c \mid \bar{T}_{i,j}, \boldsymbol{\theta})$ can be assigned to each sample \cite{BISHOP2006}. In the M stage, the parameters $\alpha_c$ and $\beta_c$ of each cluster that maximize the log-likelihood are computed by gradient descent of the CDLL \cite{NOCEDAL2006}. The corresponding derivatives are,
\begin{equation}
    \begin{split}
        \frac{\partial \mathcal{L} \left( \boldsymbol{\theta} \right)}{\partial \alpha_c} &=  \sum_{i = 1}^M \sum_{j = 1}^N \sum_{c = 1}^C \gamma_{i,j,c} \frac{\partial}{\partial \alpha_c} \log p \left( \bar{T}_{i,j} \mid \alpha_c, \beta_c \right) \\
        &= \sum_{i = 1}^M \sum_{j = 1}^N \gamma_{i,j,c} \sum_{c = 1}^C \left[ \log \bar{T}_{i,j} - \psi \left( \alpha_c \right) + \psi \left( \alpha_c + \beta_c \right) \right], \\
        \frac{\partial \mathcal{L} \left( \boldsymbol{\theta}_c \right)}{\partial \beta_c} &= \sum_{i = 1}^M \sum_{j = 1}^N \sum_{c = 1}^C \gamma_{i,j,c} \left[
        \frac{\partial}{\partial \beta_c} \log p \left( \bar{T}_{i,j} \mid \alpha_c, \beta_c \right) \right] \\
        &= \sum_{i = 1}^M \sum_{j = 1}^N \gamma_{i,j,c} \sum_{c = 1}^C \left[ \log \left( - \bar{T}_{i,j} \right)- \psi \left( \beta_k \right) + \psi \left( \alpha_c + \beta_c \right) \right].
    \end{split}
\end{equation} 
where $\partial \mathrm{B} ( \alpha_c, \beta_c ) / \partial \alpha_c  = \mathrm{B} ( \alpha_c, \beta_c ) \cdot [ \psi ( \alpha_c ) - \psi ( \alpha_c + \beta_c ) ]$, and $\psi ( \cdot )$ is the digamma function, which is $\psi ( \alpha_c ) = \Gamma^\prime ( \alpha_c ) / \Gamma \left( \alpha_c \right)$.

The optimal priors are found by maximizing the CDLL with respect to $\pi_c$, constrained to $\sum_c\pi_c=1$. As a result, the optimal priors are
\begin{equation}
    \pi_c = \frac{1}{MN}\sum_{i = 1}^M \sum_{j = 1}^N \gamma_{i,j,c}.
\end{equation}

The cloud average heights in a frame are computed using the posterior probabilities $\gamma_{i,j,c}$ in a frame, but only in the pixels with a cloud,
\begin{equation}
    \hat{H}_c = \frac{\sum_{i,j} \gamma_{i,j,c} \cdot H_{i,j} \cdot \mathbb{I} \left( b_{i,j} = 1 \right)}{\sum_{i,j} \gamma_{i,j,c} \cdot \mathbb{I} \left( b_{i,j} = 1 \right)},
\end{equation}
where $\mathbb{I} \left( \cdot \right)$ is the indicator function. An image segmentation algorithm indicates which pixels belong to a cloud, so that $\mathbf{B} = \{ b_{i,j} \in \mathbb{B} \mid \forall i = 1, \ldots, M, \ \forall j = 1, \ldots, N \}$ is a binary image where 0 is a clear sky pixel, and 1 is a pixel belonging to a cloud \cite{TERREN2020c}. 

The performance of a Gamma Mixture Model and a BeMM were compared to infer the distribution of the temperatures and the heights. The BeMM of the temperature of the pixels was found to be better when identifying which pixels belong to the wind velocity layer.

\subsubsection{Weighted Lucas-Kanade}

%In current computer vision literature, there are three primary methods to estimate the motion of objects in a sequence of images: Lucas-Kanade \cite{LUCAS1981}, Horn-Schunk \cite{HORN1981}, and Farneb{\"a}ck \cite{FERNEBACK2003}. These three methods are based on the space-time partial derivatives between two consecutive frames. Taking a different disciplinary approach, the velocity field in experimental fluid dynamics is approximated applying research methods based on signal cross-correlation operated in the frequency domain \cite{ADRIAN2011}. 

The techniques to estimate the motion vectors in an image are sensitive to the intensity gradient of the pixels. We implemented a model that removes the gradient produced by the solar direct radiation, and atmospheric scattered radiation, both of which routinely appear on the images in the course of the year. A persistent model of the outdoor germanium window of the camera removes sporadic debris that appears in the images such as water stains or dust particles \cite{TERREN2020a}.

%A series of sequences of images with clouds flowing in different directions were simulated to cross-validate the set of parameters for each one of the mentioned methods. The investigation searched for a dense implementation of a motion vector method to approximate the dynamics of clouds. 

The most suitable method was found to be the Weighted Lucas-Kanande (WLK) \cite{SIMON2003}. The weights $\gamma_{i,j,c}$ are the posterior probabilities of the BeMM. Therefore, a pixel has a velocity vector for each cloud layer $c$ in a frame. The optimal window size, weighted least-squares regularization, and differential kernel amplitude are: $\mathcal{W} = 16 [ \mathrm{pixels}^2 ]$, $\tau = 1 \times 10^{-8}$, and $\sigma = 1$ respectively. The velocity components in the x-axis are ${\bf U}_c = \{ \text{u}_{i,j,c} \in \mathbb{R} \mid \forall i = 1, \ldots, M, \ \forall j = 1, \ldots, N \}$, and  the velocity components in the y-axis are ${\bf V}_c = \{ \text{v}_{i,j,c} \in \mathbb{R} \mid \forall i = 1, \ldots, M, \ \forall j = 1, \ldots, N \}$. The velocity vectors are in units of pixels per frame, but knowing the geometrical transformation of the frame, they can be transformed to meters per second \cite{TERREN2020a}. The geometric transformation is a function of the Sun's elevation and azimuth angles $\psi : \left( \varepsilon, \alpha \right) \mapsto \Delta \mathbf{x}_{i,j} $ in a frame, it defines the dimensions of a pixel at a given height $ \Delta \mathbf{X} = \{ \left(\Delta x, \Delta y \right)_{i,j} \mid\forall i = 1, \ldots, M, \ \forall j = 1, \ldots, N \}$. This transformation connects the x,y-axis coordinates system with the height, which is the z-axis. The relation holds even when the height is an approximation, since the components of velocity vectors are transformed with respect to the new coordinates system. The velocity vectors of each cloud layer are transformed such as,
\begin{equation}
    \label{eq:geometric_transformation}
    \begin{split}
        u_{i,j} &= \frac{\delta}{f_r}  \cdot \Delta x_{i,j} \sum_{c = 1}^C  \hat{H}_c \cdot \gamma_{i,j,c} \cdot \text{u}_{i,j,c}  \\
        v_{i,j} &= \frac{\delta}{f_r} \cdot \Delta y_{i,j} \sum_{c = 1}^C \hat{H}_c \cdot \gamma_{i,j,c} \cdot \text{v}_{i,j,c}
    \end{split}s
\end{equation}
where $f_r$ is the frame rate of the sequence of images, and $\delta$ is velocity vectors' scale in the WLK approximation.

\subsection{Velocity Vectors Selection}

In order to approximate the potential lines and streamlines of the wind velocity field in a frame, we propose to select the most consistent velocity vectors over a sequence of consecutive frames. The main problems with this approach are that as the vectors are selected over a sequence of images, the amount of vectors is expected to be large; also when optical flow is implemented in dense manner, it yields to noisy vectors. Because of this, we threshold the velocity vectors to reduce both the algorithm's computational burden and the variance of the noise.

\subsubsection{Velocity Vector Segmentation}

The pixel intensity difference between two consecutive frames is computed to find the pixels that show a change. The pixel normalized intensities that were used to compute the velocity vectors are ${\mathbf{I}} = \{ {i}_{i,j} \in \mathbb{R}^{[0, 2^8)} \mid \forall i = 1, \ldots, M, \ \forall j = 1, \ldots, N \}$. The root squared intensity normalized difference is,
\begin{equation}
    {d}_{i,j} =\frac{ \sqrt{\left({i}^{k - 1}_{i,j} - {i}^k_{i,j}\right)^2}}{\sum_{i,j}{ \sqrt{\left({i}^{k - 1}_{i,j} - {i}^k_{i,j}\right)^2}}}.
\end{equation}

Matrix ${\bf D}$ with normalized differentials $d_{i,j}$ is vectorized and sorted from the lowest to the highest, i.e., ${\mathbf{d}} = \mathrm{sort}(\mathrm{vec} ({\mathbf{D}} ))$. A vector $\bf r$ with the accumulated variance is computed as
\begin{equation}
    r_m = \left\{ \sum^m_{i = 1} {\bf d}_i \right\}^{N \cdot M}_{m = 1}.
\end{equation}
Then, vector $\mathbf{r}$ is reorganized and set in the original matrix form, defined as $\mathbf{R} = \{ r_{i,j} \in \mathbb{R}^{[0,1)} \mid \forall i = 1, \dots, M, \ \forall j = 1, \dots, N \}$. Finally, a threshold $\tau$ is applied
\begin{equation}
    \label{eq:threshold}
    b_{i,j} = 
    \begin{cases}
        1 \quad r_{i,j} \geq \tau \\
        0 \quad \mathrm{Otherwise},
    \end{cases}
\end{equation}
where  $\mathbf{B} \in \mathbb{B}$ is a binary image whose elements are 1 when a pixel is selected. The threshold velocity vectors in a frame $k$ are ${{\bf V}'}^{k} = \{ \mathbf{v}^k_{i,j}=\{u_{i,j}^k,v_{i,j}^k\}  \wedge b^k_{i,j} = 1 \mid \forall i = 1, \ldots M, \ \forall j = 1, \ldots, N \}$.

Based on the assumption that a cloud floating in the air follows a trajectory dictated by the wind velocity field, the wind velocity field is approximated using the segmented velocity vectors of $\ell$ last frames. Hence, the set of velocity vectors available to compute the wind velocity field are,
\begin{equation}
    \label{eq:dataset}
    \tilde{\mathbf{V}}^{k} = \left[ {\begin{array}{ccc}
       {{\bf V}'}^k \\
       \vdots \\
       {{\bf V}'}^{k - \ell} \\
      \end{array} } \right] \in \mathbb{R}^{2 \times N^k},
\end{equation}
the number of samples in $\tilde{\mathbf{V}}^k$ is $N^k$, this number is not the same in each frame $k$. 

\subsubsection{Velocity Vector and Height Distributions}

A velocity vector $\tilde{\mathbf{v}}_i$ (by omitting superindex $k$) in the set $\tilde{\mathbf{V}}^k = \{ \tilde{\mathbf{v}}^k_i \in \mathbb{R}^2 \mid \forall i = 1, \dots, N^k\}$ is assumed to belong to a cloud layer $c$. The probability of a vector to belong to a cloud layer $c$ is modelled as an independent normal random variable $\tilde{\mathbf{v}}_i \sim \mathcal{N}( \boldsymbol{\mu}_c, \boldsymbol{\Sigma}_c )$. The function of the multivariate normal distribution is,
\begin{equation}
    p \left( \tilde{\mathbf{v}}_i \mid  \boldsymbol{\mu}_c, \boldsymbol{\Sigma}_c \right) = \frac{\mathrm{e}^{\left\{ - \frac{1}{2} \left( \tilde{\mathbf{v}}_i - \boldsymbol{\mu}_c \right)^\top \boldsymbol{\Sigma}_c^{-1} \left( \tilde{\mathbf{v}}_i- \boldsymbol{\mu}_c \right) \right\}}}{\sqrt{ \left(2 \pi\right)^d \left| \boldsymbol{\Sigma}_c \right| }}.
\end{equation}
In the case when two cloud layers were detected, we propose to infer the probability distribution of velocity vectors' in each cloud layer with this model,
\begin{equation}
    p \left( \tilde{\mathbf{v}}_i \mid \boldsymbol{\Theta} \right) \propto p \left( \tilde{\mathbf{v}}_i \mid \boldsymbol{\mu}_1, \boldsymbol{\Sigma}_1 \right)^{\lambda_i} \cdot  p \left( \tilde{\mathbf{v}}_i  \mid \boldsymbol{\mu}_2, \boldsymbol{\Sigma}_2 \right)^{\left(1 - \lambda_i \right)},
\end{equation}
where $\boldsymbol{\Theta} = \{ \boldsymbol{\lambda}, \boldsymbol{\mu}_1, \boldsymbol{\Sigma}_1, \boldsymbol{\mu}_2, \boldsymbol{\Sigma}_2\}$, and $\lambda_i \in \{0, 1\}$.  $\lambda_{i,c}$ is defined as convex, considering that a velocity vector may belong to one or the other wind velocity layer, but no to both. Knowing the vectors that belong to the first cloud layer, the vectors that belong to the second cloud layer are also known, $\lambda_{i,2} = 1 - \lambda_{i,1}$. The lower bound of the data log-likelihood is found applying Jensen's inequality \cite{JENSE1906},
\begin{equation}
	\label{eq:velocity_vectors_distribution}
    \log p \left( \tilde{\mathbf{v}}_i \mid {\boldsymbol{\Theta}} \right) \propto \lambda_{i,1} \cdot \log p \left( \tilde{\mathbf{v}}_i \mid {\boldsymbol{\mu}}_1, {\boldsymbol{\Sigma}}_1 \right) + \lambda_{i,2} \cdot \log p \left( \tilde{\mathbf{v}}_i  \mid {\boldsymbol{\mu}}_2, {\boldsymbol{\Sigma}}_2 \right),
\end{equation}
so that the posterior distribution is a linear combination of the multivariate normal distributions.

The probabilistic model parameters are inferred using a fixed-point variation of the Iterated Conditional Modes (ICM) \cite{BESAG1986}. The algorithm begins by randomly assigning the velocity vectors to a cloud layer, $\lambda_{i,1} \sim \mathcal{U} ( 0, C - 1 )$. The parameters of velocity vector distributions, in Eq. \eqref{eq:velocity_vectors_distribution} that maximize the data log-likelihood are computed in the first step of the algorithm. These same parameters are used to initialize the inference of the parameters of the height distributions in the second step in Eq. \eqref{eq:height_distributions}. 

In the case of a multivariate normal distribution, the ICM algorithm is iteratively updates parameters. At iteration $t+1$, the means and covariances are,
\begin{equation}
    \label{eq:parameters_estimation}
    {\boldsymbol{\mu}}_c^{(t + 1)} = \frac{\sum_i \lambda_{i,c}^{(t)} \cdot \tilde{\mathbf{v}}_i }{\sum_i \lambda_{i,c}^{(t)}}; \ \ \
    {\boldsymbol{\Sigma}}_c^{(t + 1)} = \frac{\sum_{i} \lambda_{i,c}^{(t)} \cdot \left( \tilde{\mathbf{v}}_i  - {\boldsymbol{\mu}}_c^{(t + 1)} \right)^\top \left( {\mathbf{v}}_i  - \tilde{\boldsymbol{\mu}}_c^{(t + 1)} \right)}{\sum_i \lambda_{i,c}^{(t)}}
\end{equation}
The vectors are re-assigned to a cloud layer at the end of each parameters update, applying the maximum a posteriori (MAP) criterion
\begin{equation}
    \begin{split}
        \lambda_{i,2}^{(t + 1)} &= \underset{c}{\operatorname{argmax}} \ p \left( \tilde{\mathbf{v}}_i \mid {\boldsymbol{\mu}}_c^{(t + 1)}, {\boldsymbol{\Sigma}}_c^{(t + 1)} \right) - 1 \\
        \lambda_{i,1}^{(t + 1)} &= 1 - \lambda_{i,2}^{(t + 1)}.  
    \end{split}
\end{equation}
After completing the inference of the velocity vectors distribution, it is possible to infer the cloud layer's height using the same method. The velocity vectors in an image were calculated using the WLK method. The algorithm approximates the velocity vector using a set of pixels inside a window. The result is that the velocity vectors do not exactly correspond to a clouds' pixels, which are in motion. Instead, the velocity vectors are assigned to nearby pixels. To identify which layer of clouds $c$, is the highest and which one is the lowest, the height distribution of the pixels is inferred using the MAP classification of the velocity vectors $\mathbf{v}^\prime_{i,j}$ in a image. 

The height of the pixels within the cloud are modelled as independently distributed normal random variables $H_{i,j} \sim \mathcal{N} (\mu_c, \sigma^2_c) $. The probabilistic model to infer the distribution of heights of each cloud layer in a frame is,
\begin{equation}
	\label{eq:height_distributions}
    \log p \left( H_{i,j} \mid \boldsymbol{\Theta} \right) \propto \rho_{i,j,1} \cdot \log p \left( H_{i,j} \mid \mu_1, \sigma^2_1 \right) + \rho_{i,j,2} \cdot \log p \left( H_{i,j} \mid \mu_2, \sigma^2_2 \right),
\end{equation}
where $\boldsymbol{\Theta} = \{\boldsymbol{P}, \mu_1, \sigma_1, \mu_2, \sigma_2 \}$, and $\rho_{i,j,c} \in \{0, 1\}$ is a convex variable so that $\rho_{i,j,2} = 1 - \rho_{i,j,1}$.

The ICM algorithm is also used to the infer the parameters of the height distributions model. The $\rho_{i,j,c}$ are initialized to the MAP classification of the velocity vectors $\mathbf{v}^\prime_{i,j}$ using the parameters that were inferred using all the velocity vectors $\tilde{\mathbf{v}}_i$ in Eq. \eqref{eq:dataset},
\begin{equation}
    \begin{split}
        \rho_{i,j,2} &= \underset{c}{\operatorname{argmax}} \ p \left( \mathbf{v}^{\prime}_{i,j} \mid \boldsymbol{\mu}_c, \boldsymbol{\Sigma}_c \right) - 1\\
    \rho_{i,j,1} &= 1 - \rho_{i,j,2}.   
    \end{split}
\end{equation}
The parameters of the height distributions are updated using the formulas in Eq. \eqref{eq:parameters_estimation}. The algorithm eventually converges so that the pixels in the frame are segmented where a cloud appears. The segmentation is performed according to the MAP classification of height distributions,
\begin{equation}
    \begin{split}
        \rho_{i,j,2}^{(t + 1)} &= \underset{c}{\operatorname{argmax}} \ p \left( H_{i,j} \mid \mu_c^{(t + 1)}, \sigma_c^{2(t + 1)}\right) - 1\\
        \rho_{i,j,1}^{(t + 1)} &= 1 - \rho_{i,j,2}^{(t + 1)}. 
    \end{split}
\end{equation}
In order to find the height of a given cloud layer, the heights are averaged with this formula,
\begin{equation}
    \bar{H}_c = \frac{\sum_{i,j} \rho_{i,j,c} \cdot H_{i,j} \cdot \mathbb{I} \left( b_{i,j} = 1 \right)}{\sum_{i,j} \rho_{i,j,c} \cdot \mathbb{I} \left( b_{i,j} = 1 \right)}.
\end{equation}
The wind velocity fields are organized into upper and lower layers by average height $\bar{H}_c$. In this way, each detected wind velocity field has a distribution of velocity vectors, and another distribution of heights.

\subsubsection{Sampling}

In order to reduce the computational burden of the algorithm, a subset of the velocity vectors is selected according to the estimated probability distributions of the vectors. At each layer $c$, we define the importance weights $w_{i,c}^k$ as
\begin{equation}
    w^k_{i,c} \triangleq p \left( \tilde{\mathbf{v}}^k_i \middle| \boldsymbol{\theta}_c \right), \quad w_{i,c}^k \in \mathbb{R}^+.
\end{equation}
The weights are normalized to have the characteristics of a probability mass function such as $\sum_{i = 1}^{N_k} \hat w_{i,c}^k = 1$. 

The Cumulative Probability Function (CDF) is computed as
\begin{equation}
    \tilde{w}^k_{i,c} = \left\{ \sum_{m = 1}^i \hat{w}^k_{m,c} \right\}_{i = 1}^{N^k}.
\end{equation}
In order to select samples for each distribution $p ( \tilde{\mathbf{v}}^k_i \mid \boldsymbol{\theta}_c )$, $N^*/C$ samples are drawn from a uniform distribution,
\begin{equation}
    z_{j,c}^k \sim \mathcal{U}\left( 0, 1 \right), \quad j = 1, \ldots, \frac{N^*}{C},
\end{equation}
For each value $z_{j,c}^k$, a sample is selected with the criterion 
\begin{equation}
    I_{j,c}^k = \operatorname{argmin} \ \mid \tilde{w}_{i,c}^k - z_{j,c}^k \mid, \ \forall i = 1, \ldots, N_k \ \forall j = 1, \ldots, \frac{N^*}{C}.
\end{equation}
The selected vectors are the ones whose CDF is closest to the values of the uniform samples $z_{j,c}^k$,
\begin{equation}
    \tilde{\mathbf{v}}_c^{*k} \triangleq \tilde{\mathbf{v}}^k_{I_{j,c}^k}, \quad \forall j = 1, \ldots, \frac{N^*}{C}.
\end{equation}

The subset of selected velocity vectors in frame $k$ for the cloud layer $c$ is $\mathbf{V}_c^{*k} = \{ ( \tilde{u}, \tilde{v} )_{j,c}^{*k} \in \mathbb{R}^2 \mid \forall j = 1, \ldots, N^*/C \} $, the subset of Euclidean coordinate pairs of those selected vectors is $\mathbf{X}_c^{*k} = \{ ( x, y )_{j,c}^{*k} \in \mathbb{N}^2 \mid \forall j = 1, \ldots, N^*/C \}$. 

Assuming that the prior is uniform, the posterior probabilities are,
\begin{equation}
    \label{eq:posterior_proba}
    z_{i,c}^{*k} \triangleq \frac{p \left( \tilde{\mathbf{v}}^{*k}_i \middle| \boldsymbol{\theta}_c \right)}{\sum_{c = 1}^C p \left( \tilde{\mathbf{v}}^{*k}_i \middle| \boldsymbol{\theta}_c \right)}.
\end{equation}

The sampling is repeated for as many cloud layers detected. All selected subsets of vectors, coordinate pairs, and weights form the dataset that is used to approximate the wind velocity field, 
\begin{equation}
    \label{eq:selected_dataset}
    \mathbf{X}^{*k} = 
      \begin{bmatrix}
        x^{*k}_1 & y^{*k}_1 \\
        \vdots & \vdots  \\
        x^{*k}_{N^*} & y^{*k}_{N^*} \\
      \end{bmatrix}, \
    \mathbf{V}^{*k} = 
      \begin{bmatrix}
        \tilde{v}^{*k}_1 & \tilde{u}^{*k}_1 \\
        \vdots & \vdots  \\
        \tilde{v}^{*k}_{N^*} & \tilde{u}^{*k}_{N^*} \\
      \end{bmatrix}, \
    \mathbf{Z}^{*k} = 
      \begin{bmatrix}
        z^{*k}_{1,1} & z^{*k}_{1,c} \\
        \vdots & \vdots  \\
        z^{*k}_{N^*,1} & z^{*k}_{N^*,c} \\
      \end{bmatrix},
\end{equation}
where $N^k >> N^*$. 

\section{Flow Visualization}

The atmosphere is a system where the dynamics are continuously changing \cite{KALNAY2003}. This fact implies that a wind velocity field exists, but we can only visualize it where clouds are present. From ground level to the Tropopause, the wind flow can have multiple layers with different velocities in each one of the layers. The wind flow may also be convective, however, for the sake of simplicity, we assume that the multi-layer flow which is observed in IR images is a multi-layer laminar flow. This analysis neither considers the z-component in the motion of a cloud (which is not observable)  nor the possible inter-crossing of cloud layers.

\subsection{Wind Velocity Field Estimation}

Three methods were implemented to estimate the extrapolation function and compare their performances. The first method uses a weighted $\varepsilon$-support vector regression machine  ($\varepsilon$-WSVM) for each one of the velocity components. The second method is a $\varepsilon$-MO-WSVM that estimates both velocity components. The third is an innovation which uses a $\varepsilon$-MO-WSVM with flow constraints ($\varepsilon$-MO-WSVM-FC) to estimate both velocity components. The flow constraints are used to force the extrapolated wind flow to have zero divergence or curl, so it can be assumed that, in the approximated wind flow, streamlines are equivalent to the cloud pathlines.

The regression problem can be formulated as the optimization of a function with the form,
\begin{equation}
    f \left(\mathbf{x}_i\right) = \mathbf{w}^\top \varphi \left( \mathbf{x}_i \right) + b, \ \forall i = 1, \dots, N^*, \ \mathbf{w}, \mathbf{x}_i \in \mathbb{R}^D,\ b \in \mathbb{R}.
\end{equation}
where $\mathbf{x}_i \triangleq \mathbf{x}^{*k}_i$  in our problem, and where $\varphi(\cdot)$ is a transformation into a higher dimensional (possibly infinite) Hilbert space $\mathcal{H}$ endowed with a dot product $\mathcal{K}({\bf x}_i,{\bf x}_j)=\langle \varphi({\bf x}_i),\varphi({\bf x}_j)$. A function  $\mathcal{K}({\bf x}_i,{\bf x}_j)$ is a dot product if it is a bivariate positive semi-definite function that maps ${\bf x}_i,{\bf x}_j$ into $\mathbb{R}$, commonly called a Mercer's kernel or simply a kernel function. 

\subsubsection{Support Vector Machine for Regression}

Assuming $\mathbf{v}_i =\{u_i,v_i\} \triangleq \mathbf{v}_i^{*k}$, the regression problem in a $\varepsilon$-SVM is formulated with an $\varepsilon$-insensitive loss function, which penalizes the errors $ |\varepsilon| > 0$ \cite{DRUCKER1997} for each one of the components in ${\bf v}_i$ and for each cloud layer $c$ as
\begin{equation}
    \left| u_i - f \left( \mathbf{x}_i \right)\right|_{\varepsilon} = \max \left[ 0, \left| u_i - f \left( \mathbf{x}_i \right)\right|-\varepsilon \right], \ \forall i = 1, \dots, N, \ u_i,\varepsilon \in \mathbb{R},
\end{equation}
and identically for $v_i$. The $\varepsilon$-insensitive loss function can be seen as a tube of radius $\varepsilon$ adjusted around the regression hyper-plane via the Support Vectors (SV) \cite{SCHOLKOPF2000}.

The samples are weighted by their probability of belonging to wind velocity field $c$ \cite{ELATTAR2010},
\begin{equation}
    \begin{split}
        z_i &\triangleq z_i^{*k}, \quad z_i \in \mathbb{R}^{\leq 1}. \\
        c_i &= z_i \cdot \frac{C}{N}       
    \end{split}
\end{equation}
The L2-norm and $\varepsilon$-loss function is applied to the model weights, 
\begin{equation}
    \label{eq:primal}
    \begin{split}
    \min_{\mathbf{w}, b, \xi, \xi^*} & \quad \frac{1}{2} \| \mathbf{w} \|^2 + \frac{C}{N} \sum_{i = 1}^N z_i \left( \xi_i + \xi_i^* \right) \\ 
    \mathrm{s.t.} & 
    \begin{cases}
        u_{i}-\mathbf{w}^\top \varphi \left( \mathbf{x}_i \right) - b & \leq \varepsilon + \xi_i \\
        \mathbf{w}^\top \varphi \left( \mathbf{x}_i \right) + b  - u_{i} & \leq \varepsilon + \xi_i^* \\
        \xi_i, \xi_i^* & \geq 0
    \end{cases}  \quad i = 1, \ldots, N, 
    \end{split}
\end{equation}
and identically for $v_i$. The slack variables $\xi_i$ were introduced to relax the constraints of the optimization problem and to deal with unfeasible optimization problems \cite{CORTES1995}. The primal objective function aims to find the trade off between the regularization term $\varepsilon$, the allowed errors or slack variables $\xi_i$ and $\xi_i^*$, and the complexity of the model $c_i$ per weighted sample.

The proposed kernel functions in this analysis are, 
\begin{equation}
    \begin{split}
        \mathcal{K} \left( \mathbf{x}_i, \mathbf{x}_j \right) &= \mathbf{x}_i^\top \mathbf{x}_j, \\ 
        \mathcal{K} \left( \mathbf{x}_i, \mathbf{x}_j \right) &= \exp \left( - \gamma \cdot || \mathbf{x}_i - \mathbf{x}_j ||^2 \right), \\
        \mathcal{K} \left( \mathbf{x}_i, \mathbf{x}_j \right) &= \left( \gamma \cdot \mathbf{x}_i^\top \mathbf{x}_j + \beta \right)^d,        
    \end{split}
\end{equation}
where $\gamma, \ \beta \in \mathbb{R}$, and $d \in \mathbb{N}$ are the kernel hyperparameters that need cross-validation. \cite{SCHOLKOPF2000}. These kernel functions are referred to as linear, radial basis function (RBF) or square exponential, and polynomial of order $d$ respectively \cite{SHAWE2004}.

In order to optimize the constrained problem in functional \eqref{eq:primal} and constraints \eqref{eq:primal_constraints} a Langrangian functional is constructed with the functional and the set of constraints through a dual set of new variables \cite{SMOLA2004}, which leads to a solvable Quadratic Programming problem (QP). The Lagrangian functional is 
\begin{equation}
    \begin{split}
        \mathcal{L} & \left( \mathbf{w}, b,\alpha, \alpha^*, \beta, \xi, \xi^*, \varepsilon, \eta, \eta^* \right) = \\
        & = \frac{1}{2} \| \mathbf{w} \|^2 + c_i \sum_{i = 1}^N \left( \xi_i + \xi_i^* \right) \ \ldots \\
        & - \sum_{i = 1}^N \left( \eta_i \xi_i + \eta_i^* \xi_i* \right) - \sum_{i = 1}^N \alpha_i \left( \varepsilon + \xi_i - u_i + \mathbf{w}^\top \varphi \left( \mathbf{x}_i \right) + b \right) \ \ldots \\
        & - \sum_{i = 1}^N \alpha_i^* \left( \varepsilon + \xi_i^* + u_i -  \mathbf{w}^\top \varphi \left( \mathbf{x}_i \right)- b \right), \quad \forall i = 1, \dots, N, \quad \eta_i, \eta_i^* \in \mathbb{R}.  
    \end{split}
\end{equation}
The derivatives of the primal variables $\mathbf{w},\varepsilon, \xi_i, \xi_i^*$  yield to the following set of equations, which is a case of Karush-Kuhn-Tucker (KKT) conditions,
\begin{equation}
    \begin{split}
        \mathbf{w}^\top &= \sum_{i = 1}^N \left( \alpha_i^* - \alpha_i \right) \varphi \left( \mathbf{x}_i \right), \\
        0 &= \sum_{i = 1}^N \left( \alpha_i - \alpha_i^* \right ), \\
        0 &= c_i - \alpha_{i} - \eta_{i}, \\
        0 &= c_i 
        - \alpha_{i}^* - \eta_{i}^*.
    \end{split}
\end{equation}
These conditions, together with the complimentary KKT conditions (which force the product of dual parameters $\alpha_i,\alpha^*_i$ with the constraints to be zero) leads to the following dual functional by substitution on the Lagrangian: 
\begin{equation}
    \begin{split}
        \min_{\boldsymbol{\alpha}, \boldsymbol{\alpha}^*} &\quad \frac{1}{2} \cdot \left( \boldsymbol{\alpha} - \boldsymbol{\alpha}^* \right)^\top \mathbf{K} \left( \boldsymbol{\alpha} - \boldsymbol{\alpha}^* \right) + \sum_{i=1}^N \left( {\alpha_i} - \alpha_i^* \right)u_i + \varepsilon \cdot  \mathbf{1}^\top \left( \boldsymbol{\alpha} + \boldsymbol{\alpha}^* \right) \\
        &\mathrm{s.t.}
        \begin{cases} 
            \mathbf{1}^\top \left( \boldsymbol{\alpha} - \boldsymbol{\alpha}^* \right) = 0 \\ 
            0 \leq \alpha_i, \alpha_i^* \leq c_i
        \end{cases} \ \forall i = 1, \dots, N.   
    \end{split}
\end{equation}
where $\mathbf{1}_{1 \times N} = [1, \ldots, 1 ]^\top$, and matrix $\bf{K}$ is a Gram matrix of dot product such that ${\bf K}_{i,j} = \mathcal{K}({\bf x}_i,{\bf x}_j) $. The minimal of the primal function is equivalent to the saddle point on the Lagrangian formulation. The approximated function is,
\begin{equation}
    f \left( \mathbf{x} \right) = \sum_{i = 1}^N  \left(\alpha_i  - \alpha^*_{i}\right) \cdot \mathcal{K} \left( \mathbf{x}_i, \mathbf{x}_i \right) + b,
\end{equation}
where $b$ is obtained from the complimentary KKT conditions. 

\subsubsection{Multi-Ouput Weighted Support Vector Machine}

When the wind velocity field function is approximated by $\varepsilon$-MO-SVM,the primal regression can be formulated as 
\begin{equation}
    {\bf v}_i = {\bf W}^\top\varphi({\bf x}_i)+{\bf b},
\end{equation}
where each one of the column vectors of primal parameter matrix ${\bf W}$ approximates one of the velocities in vector ${\bf y}_i$. Primal parameters are a function of the dual parameters as well, but the dual parameters $\boldsymbol{\alpha}_i, \boldsymbol{\alpha}_i^{*}$ are vectors in a $2$-dimensional multi-output problem. 

Since independent variables are represented in vectors ${\bf v}_i$, the training set is defined in a vector  $\tilde{\mathbf{v}}_{1 \times 2N}$, and so are the dual parameters $\tilde{\boldsymbol{\alpha}}_{1 \times 2N}$ and $\tilde{\boldsymbol{\alpha}}^*_{1 \times 2N} $ for notation simplicity.

The gram matrix of dot products between input patterns $\varphi({\bf x}_i)$ can be interpreted as the covariance matrix between variables ${\bf v}_i$. Indeed
\begin{equation}
    \begin{split}
        \mathbb{E}\left(({\bf v}_i-{\bf b}^\top)({\bf v}_j-{\bf b})\right) &= \mathbb{E}\left(   {\bf W}^\top \varphi({\bf x}_i) \varphi({\bf x}_j)^\top{\bf W}\right) \\
        &= \left( \begin{array}{cc}
        \varphi({\bf x}_i)^\top \Sigma_{11} \varphi({\bf x}_j)&\varphi({\bf x}_i)^\top \Sigma_{12}\varphi({\bf x}_j)\\
        \varphi({\bf x}_i)^\top \Sigma_{21}\varphi({\bf x}_j)&\varphi({\bf x}_i)^\top \Sigma_{22}\varphi({\bf x}_j)\\
        \end{array} \right),
    \end{split}
\end{equation}
where the $2\times2$ covariance $ \mathbb{E}\left({\bf W}{\bf W}^\top\right) $ is interpreted as a model for the dependencies between elements in ${\bf v}_i$, i.e. 
\begin{equation}
    \mathbb{E}\left({\bf W}{\bf W}^\top\right)=
    \left(\begin{array}{cc}
    \Sigma_{11} & \Sigma_{12}\\
    \Sigma_{21} & \Sigma_{22}
    \end{array}\right).
\end{equation}

If we consider that both vertical and horizontal velocities are independent, then $\Sigma_{12}=\Sigma_{21}={\bf 0}$. If we assume further that $\Sigma_{11}=\Sigma_{22}={\bf I}$ for simplicity, which, in turn leads to
\begin{equation}
    \mathbb{E}\left(({\bf v}_i-{\bf b}^\top)({\bf v}_j-{\bf b})\right) =
    \left(\begin{array}{cc}
    \mathcal{K}({\bf x}_i,{\bf x}_j)&0\\
    0&\mathcal{K}({\bf x}_i,{\bf x}_j)\\
    \end{array}\right).
\end{equation}

The Gram matrix $\tilde{\mathbf{K}}_{DN \times DN}$ in the $\varepsilon$-MO-SVM formulation for independent components is,
\begin{equation}
    \tilde{\mathbf{K}} = \left( \begin{array}{cc}
        \mathbf{K} & \mathbf{0} \\ 
        \mathbf{0} & \mathbf{K}
    \end{array} \right).
\end{equation}
The full kernel matrix in a $\varepsilon$-MO-WSVM is computationally expensive, and it is not implemented in this research.

The extension of weights in the $\varepsilon$-MO-WSVM requires weighting each sample in each output \cite{HAN2014}, 
\begin{equation}
    \begin{split}
        \tilde{z}_i &= \left[ z \ldots z_N \ z_1 \ldots z_N \right]^\top, \quad
        \sum_{i = 1}^{D \cdot N} \tilde{z}_i = 2, \quad \tilde{z}_i \in \mathbb{R}^{\leq 1}.
    \end{split}
\end{equation}

The dual formulation of the QP problem for the $\varepsilon$-MO-WSVM is,
\begin{equation}
    \label{eq:dual_formaulation}
    \begin{split}
        \min_{\tilde{\boldsymbol{\alpha}}, \tilde{\boldsymbol{\alpha}}^*} & \quad \frac{1}{2} \cdot \left( \tilde{\boldsymbol{\alpha}} - \tilde{\boldsymbol{\alpha}}^* \right)^\top \tilde{\mathbf{K}} \left( \tilde{\boldsymbol{\alpha}} - \tilde{\boldsymbol{\alpha}}^* \right) + \tilde{\mathbf{y}}^\top \left( \tilde{\boldsymbol{\alpha}} - \tilde{\boldsymbol{\alpha}}^* \right) + \varepsilon \cdot \mathbf{1}^\top \left( \tilde{\boldsymbol{\alpha}} + \tilde{\boldsymbol{\alpha}}^* \right) \\
        &\mathrm{s.t.}
        \begin{cases} 
            \mathbf{1}^\top \left( \tilde{\boldsymbol{\alpha}} - \tilde{\boldsymbol{\alpha}}^* \right) = 0 \\ 
            \mathbf{0} \leq \tilde{\alpha}_i, \tilde{\alpha}_i^* \leq \tilde{c}_i \\
        \end{cases}  \ \forall i = 1, \dots, 2 N,  
    \end{split}
\end{equation}
where the extended weighted complexity is $\tilde{c_i} = \tilde{z}_i / 2N$.

\subsubsection{Multi-Ouput Weighted Support Vector Machine with Flow Constraints}

Assuming that the analyzed air parcel is sufficiently small so that the flow can be considered approximately incompressible and irrotational, a new set of flow constraints are added to the original set of constraints with the purpose of visualizing the wind velocity field to force the divergence and the vorticity to zero:
\begin{equation}
    \label{eq:flow_constraints}
    \mathrm{s.t.}
    \begin{cases} 
        \left( \tilde{\mathbf{v}}^{k\top}_c \mathbf{\Delta}_{x,y} \mathbf{\dot{V}} \right)  \cdot \left( \tilde{\mathbf{v}}^{k\top}_c \mathbf{\Delta}_{x,y} \mathbf{\dot{V}} \right)^\top &= 0 \\
        \left(  \tilde{\mathbf{v}}^{k\top}_c \mathbf{\Delta}_{x,y} \mathbf{\dot{D}} \right) \cdot \left( \tilde{\mathbf{v}}^{k\top}_c \mathbf{\Delta}_{x,y} \mathbf{\dot{D}} \right)^\top &= 0,
    \end{cases} 
\end{equation}
where the matrices of this expression are defined in Eq. \eqref{eq:matrix_1} Eq. \eqref{eq:set_matrix_1} and Eq. \eqref{eq:set_matrix_2}. To compute the vorticity and divergence, the differentiation of the velocity field along the x-axis, the and y-axis is implemented using operator
\begin{equation}
    \label{eq:matrix_1}
    \mathbf{\Delta}_{x,y} =
    \begin{bmatrix}
        \boldsymbol{\Delta}_x & \mathbf{0} \\
        \mathbf{0} & \boldsymbol{\Delta}_y
    \end{bmatrix}_{2N \times 2N},
\end{equation}
where the differential operators $\boldsymbol{\Delta}_x$ and $\boldsymbol{\Delta}_y$ are defined as,
\begin{equation}
    \label{eq:set_matrix_1}
    \boldsymbol{\Delta}_x =
    \begin{bmatrix}
        -1 & 0 & \ldots & 0\\
        1 & -1 & \ddots & \vdots \\
        0 & 1 & \ddots & 0 \\
        \vdots &  \ddots & \ddots & -1\\
        0 & \ldots & 0 & 1
    \end{bmatrix}_{N \times N}; \quad
    \boldsymbol{\Delta}_y =
    \begin{bmatrix}
        -1 & \ldots & 0 \\
        \vdots & \ddots  & \vdots  \\
        0 & \ldots & -1 \\
        1 & \ldots & 0  \\
        \vdots & \ddots & \vdots \\
        0 & \ldots & 1
    \end{bmatrix}_{N \times N}.
\end{equation}
The operators of the velocity field's vorticity and divergence are respectively,
\begin{equation}
    \label{eq:set_matrix_2}
    \mathbf{\dot{V}} = \left[ \mathbf{I} \quad \mathbf{I} \right]^\top_{2N \times N}, 
    \mathbf{\dot{D}} = \left[ \mathbf{I} \quad -\mathbf{I} \right]^\top_{2N \times N}
\end{equation}

The velocity field is extrapolated to the entire frame using the inferred parameters in frame $k$
\begin{equation}
    \label{eq:extrapolation}
    \hat{\mathbf{v}}^k_c = \left( \tilde{\boldsymbol\alpha}^k_c - \tilde{\boldsymbol\alpha}^{*k}_c \right) \cdot \mathcal{K} \left( \mathbf{X}^{*k}, \mathbf{X} \right) + \mathbf{b}_c^k,
\end{equation}
where the velocity components are $\hat{\mathbf{U}}^k_c \triangleq \hat{\mathbf{v}}^k_{x,c}$, and $\hat{\mathbf{V}}^k_c \triangleq \hat{\mathbf{v}}^k_{y,c}$, where  $\hat{\mathbf{U}}_c^k, \hat{\mathbf{V}}^k_c \in \mathbb{R}^{M \times N} $. 

To compute the flow constraints, the velocity field has to be extrapolated to the whole frame using Eq. \eqref{eq:extrapolation}. The constraints in Eq. \eqref{eq:flow_constraints} are added to the constraints in the dual formulation of the $\varepsilon$-MO-SVM in Eq. \eqref{eq:dual_formaulation}. 


\section{Wind Velocity Field Streamlines}

To estimate the wind velocity field dynamics, velocity vectors are approximated using the WLK method. The velocity vectors are weighted by the posterior probabilities of the cloud layers in the image, and transformed to the cloud layer plane. The velocity vectors are segmented and sampled to reduce the noise and the computation burden. The parameters of the $\varepsilon$-MO-WSVM-FC are cross-validated, and the model is trained to estimate the wind velocity field of the detected cloud layers. If an optimal set of parameters is available, it is possible to proceed with the training of $\varepsilon$-MO-WSVM-FM without performing the cross-validation. After training the $\varepsilon$-MO-WSVM-FC, the testing is performed to extrapolate the wind velocity field to the whole image. The streamlines are computed using Eq. \eqref{eq:streamlines} to visualize the trajectory of a cloud. The potential lines are not shown in the Fig. \ref{fig:day_2_layer_0_turbulent}-\ref{fig:day_5_layer_1}, but they are computed with Eq. \eqref{eq:potential_lines}.

The physical process of cloud formation and evolution over time is part of atmospheric thermodynamics and may have divergence and vorticity \cite{LAMB2011}. The air parcel in one frame is very small compared to the whole volume of air contained in the atmosphere. Within this frame we consider it feasible that there is no vorticity or divergence, and the approximated streamlines are equivalent to the pathlines. Henceforth, the obtained results are a numerical approximation of the actual atmospheric air parcel flow.

When we assume that a flow does not have divergence and vorticity, the stream and velocity potential functions are orthogonal, and we can apply Cauchy-Riemann equations to calculate their rates of change \cite{GRANGER1995}. For the stream function we determine $d \phi = v_x dy - v_y dx$ using samples of functions. The trapezoidal rule of numerical analysis is applied to solve the definite integrals \cite{DRAGOMIR1999}. The values of a streamline are,
\begin{equation}
    \label{eq:streamlines}
    \begin{split}
        \boldsymbol{\Phi}_c &= \frac{\hat{H}_c}{2}  \left\{ \sum^i_{m = 1} \hat{\bf u}_{m,c} \odot \Delta {\bf y}_{m,c} \right\}^N_{i = 1} \\
        &- \frac{\hat{H}_c}{2}\left\{ \sum^j_{m = 1} \hat{\bf v}_{m,c} \odot \Delta {\bf x}_{m,c} \right\}^N_{j = 1} ,
    \end{split}
\end{equation}
where $\odot$ denotes the element-wise matrix multiplication. This is the sum of element-wise products between each velocity component and its opposite differential increments.

%The total change in the potential function is $d\psi = v_x dx + v_y dy$, so we can determine the potential in each pixel $\mathbf{x} = \{x, y\}$ as,
%\begin{equation}
%    \boldsymbol{\Psi}_c = \frac{\hat{H}_c}{2} \left[ \left\{ \sum^j_{m = 1} \hat{\bf u}_{m,c} \odot \Delta {\bf x}_{m,c} \right\}^N_{j = 1} + \left\{ \sum^i_{m = 1} \hat{\bf v}_{m,c} \odot \Delta {\bf y}_{m,c}  \right\}^M_{i = 1}  \right].
%\end{equation}
%the sum of each element-wise product between the velocity components, and their differential increment. 

==> summary_methods.tex <==
\subsection{Wind Velocity Field Estimation}

Three methods were implemented to estimate the extrapolation function and compare their performances. The first method uses a weighted $\varepsilon$-support vector regression machine  ($\varepsilon$-WSVM) for each one of the velocity components. The second method is a $\varepsilon$-MO-WSVM that estimates both velocity components. The third is an innovation which uses a $\varepsilon$-MO-WSVM with flow constraints ($\varepsilon$-MO-WSVM-FC) to estimate both velocity components. The flow constraints are used to force the extrapolated wind flow to have zero divergence or curl, so it can be assumed that, in the approximated wind flow, streamlines are equivalent to the cloud pathlines.

The regression problem can be formulated as the optimization of a function with the form,
\begin{equation}
    f \left(\mathbf{x}_i\right) = \mathbf{w}^\top \varphi \left( \mathbf{x}_i \right) + b, \ \forall i = 1, \dots, N^*, \ \mathbf{w}, \mathbf{x}_i \in \mathbb{R}^D,\ b \in \mathbb{R}.
\end{equation}
where $\mathbf{x}_i \triangleq \mathbf{x}^{*k}_i$  in our problem, and where $\varphi(\cdot)$ is a transformation into a higher dimensional (possibly infinite) Hilbert space $\mathcal{H}$ endowed with a dot product $\mathcal{K}({\bf x}_i,{\bf x}_j)=\langle \varphi({\bf x}_i),\varphi({\bf x}_j)$. A function  $\mathcal{K}({\bf x}_i,{\bf x}_j)$ is a dot product if it is a bivariate positive semi-definite function that maps ${\bf x}_i,{\bf x}_j$ into $\mathbb{R}$, commonly called a Mercer's kernel or simply a kernel function. 

\subsubsection{Support Vector Machine for Regression}

Assuming $\mathbf{v}_i =\{u_i,v_i\} \triangleq \mathbf{v}_i^{*k}$, the regression problem in a $\varepsilon$-SVM is formulated with an $\varepsilon$-insensitive loss function, which penalizes the errors $ |\varepsilon| > 0$ \cite{DRUCKER1997} for each one of the components in ${\bf v}_i$ and for each cloud layer $c$ as
\begin{equation}
    \left| u_i - f \left( \mathbf{x}_i \right)\right|_{\varepsilon} = \max \left[ 0, \left| u_i - f \left( \mathbf{x}_i \right)\right|-\varepsilon \right], \ \forall i = 1, \dots, N, \ u_i,\varepsilon \in \mathbb{R},
\end{equation}
and identically for $v_i$. The $\varepsilon$-insensitive loss function can be seen as a tube of radius $\varepsilon$ adjusted around the regression hyper-plane via the Support Vectors (SV) \cite{SCHOLKOPF2000}.

The samples are weighted by their probability of belonging to wind velocity field $c$ \cite{ELATTAR2010},
\begin{equation}
    \begin{split}
        z_i &\triangleq z_i^{*k}, \quad z_i \in \mathbb{R}^{\leq 1}. \\
        c_i &= z_i \cdot \frac{C}{N}       
    \end{split}
\end{equation}
The L2-norm and $\varepsilon$-loss function is applied to the model weights, 
\begin{equation}
    \label{eq:primal}
    \begin{split}
    \min_{\mathbf{w}, b, \xi, \xi^*} & \quad \frac{1}{2} \| \mathbf{w} \|^2 + \frac{C}{N} \sum_{i = 1}^N z_i \left( \xi_i + \xi_i^* \right) \\ 
    \mathrm{s.t.} & 
    \begin{cases}
        u_{i}-\mathbf{w}^\top \varphi \left( \mathbf{x}_i \right) - b & \leq \varepsilon + \xi_i \\
        \mathbf{w}^\top \varphi \left( \mathbf{x}_i \right) + b  - u_{i} & \leq \varepsilon + \xi_i^* \\
        \xi_i, \xi_i^* & \geq 0
    \end{cases}  \quad i = 1, \ldots, N, 
    \end{split}
\end{equation}
and identically for $v_i$. The slack variables $\xi_i$ were introduced to relax the constraints of the optimization problem and to deal with unfeasible optimization problems \cite{CORTES1995}. The primal objective function aims to find the trade off between the regularization term $\varepsilon$, the allowed errors or slack variables $\xi_i$ and $\xi_i^*$, and the complexity of the model $c_i$ per weighted sample.

The proposed kernel functions in this analysis are, 
\begin{equation}
    \begin{split}
        \mathcal{K} \left( \mathbf{x}_i, \mathbf{x}_j \right) &= \mathbf{x}_i^\top \mathbf{x}_j, \\ 
        \mathcal{K} \left( \mathbf{x}_i, \mathbf{x}_j \right) &= \exp \left( - \gamma \cdot || \mathbf{x}_i - \mathbf{x}_j ||^2 \right), \\
        \mathcal{K} \left( \mathbf{x}_i, \mathbf{x}_j \right) &= \left( \gamma \cdot \mathbf{x}_i^\top \mathbf{x}_j + \beta \right)^d,        
    \end{split}
\end{equation}
where $\gamma, \ \beta \in \mathbb{R}$, and $d \in \mathbb{N}$ are the kernel hyperparameters that need cross-validation. \cite{SCHOLKOPF2000}. These kernel functions are referred to as linear, radial basis function (RBF) or square exponential, and polynomial of order $d$ respectively \cite{SHAWE2004}.

In order to optimize the constrained problem in functional \eqref{eq:primal} and constraints \eqref{eq:primal_constraints} a Langrangian functional is constructed with the functional and the set of constraints through a dual set of new variables \cite{SMOLA2004}, which leads to a solvable Quadratic Programming problem (QP). The Lagrangian functional is 
\begin{equation}
    \begin{split}
        \mathcal{L} & \left( \mathbf{w}, b,\alpha, \alpha^*, \beta, \xi, \xi^*, \varepsilon, \eta, \eta^* \right) = \\
        & = \frac{1}{2} \| \mathbf{w} \|^2 + c_i \sum_{i = 1}^N \left( \xi_i + \xi_i^* \right) \ \ldots \\
        & - \sum_{i = 1}^N \left( \eta_i \xi_i + \eta_i^* \xi_i* \right) - \sum_{i = 1}^N \alpha_i \left( \varepsilon + \xi_i - u_i + \mathbf{w}^\top \varphi \left( \mathbf{x}_i \right) + b \right) \ \ldots \\
        & - \sum_{i = 1}^N \alpha_i^* \left( \varepsilon + \xi_i^* + u_i -  \mathbf{w}^\top \varphi \left( \mathbf{x}_i \right)- b \right), \quad \forall i = 1, \dots, N, \quad \eta_i, \eta_i^* \in \mathbb{R}.  
    \end{split}
\end{equation}
The derivatives of the primal variables $\mathbf{w},\varepsilon, \xi_i, \xi_i^*$  yield to the following set of equations, which is a case of Karush-Kuhn-Tucker (KKT) conditions,
\begin{equation}
    \begin{split}
        \mathbf{w}^\top &= \sum_{i = 1}^N \left( \alpha_i^* - \alpha_i \right) \varphi \left( \mathbf{x}_i \right), \\
        0 &= \sum_{i = 1}^N \left( \alpha_i - \alpha_i^* \right ), \\
        0 &= c_i - \alpha_{i} - \eta_{i}, \\
        0 &= c_i 
        - \alpha_{i}^* - \eta_{i}^*.
    \end{split}
\end{equation}
These conditions, together with the complimentary KKT conditions (which force the product of dual parameters $\alpha_i,\alpha^*_i$ with the constraints to be zero) leads to the following dual functional by substitution on the Lagrangian: 
\begin{equation}
    \begin{split}
        \min_{\boldsymbol{\alpha}, \boldsymbol{\alpha}^*} &\quad \frac{1}{2} \cdot \left( \boldsymbol{\alpha} - \boldsymbol{\alpha}^* \right)^\top \mathbf{K} \left( \boldsymbol{\alpha} - \boldsymbol{\alpha}^* \right) + \sum_{i=1}^N \left( {\alpha_i} - \alpha_i^* \right)u_i + \varepsilon \cdot  \mathbf{1}^\top \left( \boldsymbol{\alpha} + \boldsymbol{\alpha}^* \right) \\
        &\mathrm{s.t.}
        \begin{cases} 
            \mathbf{1}^\top \left( \boldsymbol{\alpha} - \boldsymbol{\alpha}^* \right) = 0 \\ 
            0 \leq \alpha_i, \alpha_i^* \leq c_i
        \end{cases} \ \forall i = 1, \dots, N.   
    \end{split}
\end{equation}
where $\mathbf{1}_{1 \times N} = [1, \ldots, 1 ]^\top$, and matrix $\bf{K}$ is a Gram matrix of dot product such that ${\bf K}_{i,j} = \mathcal{K}({\bf x}_i,{\bf x}_j) $. The minimal of the primal function is equivalent to the saddle point on the Lagrangian formulation. The approximated function is,
\begin{equation}
    f \left( \mathbf{x} \right) = \sum_{i = 1}^N  \left(\alpha_i  - \alpha^*_{i}\right) \cdot \mathcal{K} \left( \mathbf{x}_i, \mathbf{x}_i \right) + b,
\end{equation}
where $b$ is obtained from the complimentary KKT conditions. 

\subsubsection{Multi-Ouput Weighted Support Vector Machine}

When the wind velocity field function is approximated by $\varepsilon$-MO-SVM,the primal regression can be formulated as 
\begin{equation}
    {\bf v}_i = {\bf W}^\top\varphi({\bf x}_i)+{\bf b},
\end{equation}
where each one of the column vectors of primal parameter matrix ${\bf W}$ approximates one of the velocities in vector ${\bf y}_i$. Primal parameters are a function of the dual parameters as well, but the dual parameters $\boldsymbol{\alpha}_i, \boldsymbol{\alpha}_i^{*}$ are vectors in a $2$-dimensional multi-output problem. 

Since independent variables are represented in vectors ${\bf v}_i$, the training set is defined in a vector  $\tilde{\mathbf{v}}_{1 \times 2N}$, and so are the dual parameters $\tilde{\boldsymbol{\alpha}}_{1 \times 2N}$ and $\tilde{\boldsymbol{\alpha}}^*_{1 \times 2N} $ for notation simplicity.

The gram matrix of dot products between input patterns $\varphi({\bf x}_i)$ can be interpreted as the covariance matrix between variables ${\bf v}_i$. Indeed
\begin{equation}
    \begin{split}
        \mathbb{E}\left(({\bf v}_i-{\bf b}^\top)({\bf v}_j-{\bf b})\right) &= \mathbb{E}\left(   {\bf W}^\top \varphi({\bf x}_i) \varphi({\bf x}_j)^\top{\bf W}\right) \\
        &= \left( \begin{array}{cc}
        \varphi({\bf x}_i)^\top \Sigma_{11} \varphi({\bf x}_j)&\varphi({\bf x}_i)^\top \Sigma_{12}\varphi({\bf x}_j)\\
        \varphi({\bf x}_i)^\top \Sigma_{21}\varphi({\bf x}_j)&\varphi({\bf x}_i)^\top \Sigma_{22}\varphi({\bf x}_j)\\
        \end{array} \right),
    \end{split}
\end{equation}
where the $2\times2$ covariance $ \mathbb{E}\left({\bf W}{\bf W}^\top\right) $ is interpreted as a model for the dependencies between elements in ${\bf v}_i$, i.e. 
\begin{equation}
    \mathbb{E}\left({\bf W}{\bf W}^\top\right)=
    \left(\begin{array}{cc}
    \Sigma_{11} & \Sigma_{12}\\
    \Sigma_{21} & \Sigma_{22}
    \end{array}\right).
\end{equation}

If we consider that both vertical and horizontal velocities are independent, then $\Sigma_{12}=\Sigma_{21}={\bf 0}$. If we assume further that $\Sigma_{11}=\Sigma_{22}={\bf I}$ for simplicity, which, in turn leads to
\begin{equation}
    \mathbb{E}\left(({\bf v}_i-{\bf b}^\top)({\bf v}_j-{\bf b})\right) =
    \left(\begin{array}{cc}
    \mathcal{K}({\bf x}_i,{\bf x}_j)&0\\
    0&\mathcal{K}({\bf x}_i,{\bf x}_j)\\
    \end{array}\right).
\end{equation}

The Gram matrix $\tilde{\mathbf{K}}_{DN \times DN}$ in the $\varepsilon$-MO-SVM formulation for independent components is,
\begin{equation}
    \tilde{\mathbf{K}} = \left( \begin{array}{cc}
        \mathbf{K} & \mathbf{0} \\ 
        \mathbf{0} & \mathbf{K}
    \end{array} \right).
\end{equation}
The full kernel matrix in a $\varepsilon$-MO-WSVM is computationally expensive, and it is not implemented in this research.

The extension of weights in the $\varepsilon$-MO-WSVM requires weighting each sample in each output \cite{HAN2014}, 
\begin{equation}
    \begin{split}
        \tilde{z}_i &= \left[ z \ldots z_N \ z_1 \ldots z_N \right]^\top, \quad
        \sum_{i = 1}^{D \cdot N} \tilde{z}_i = 2, \quad \tilde{z}_i \in \mathbb{R}^{\leq 1}.
    \end{split}
\end{equation}

The dual formulation of the QP problem for the $\varepsilon$-MO-WSVM is,
\begin{equation}
    \label{eq:dual_formaulation}
    \begin{split}
        \min_{\tilde{\boldsymbol{\alpha}}, \tilde{\boldsymbol{\alpha}}^*} & \frac{1}{2} \left( \tilde{\boldsymbol{\alpha}} - \tilde{\boldsymbol{\alpha}}^* \right)^\top \tilde{\mathbf{K}} \left( \tilde{\boldsymbol{\alpha}} - \tilde{\boldsymbol{\alpha}}^* \right) + \tilde{\mathbf{y}}^\top \left( \tilde{\boldsymbol{\alpha}} - \tilde{\boldsymbol{\alpha}}^* \right) + \varepsilon \mathbf{1}^\top \left( \tilde{\boldsymbol{\alpha}} + \tilde{\boldsymbol{\alpha}}^* \right) \\
        &\mathrm{s.t.}
        \begin{cases} 
            \mathbf{1}^\top \left( \tilde{\boldsymbol{\alpha}} - \tilde{\boldsymbol{\alpha}}^* \right) = 0 \\ 
            \mathbf{0} \leq \tilde{\alpha}_i, \tilde{\alpha}_i^* \leq \tilde{c}_i \\
        \end{cases}  \ \forall i = 1, \dots, 2 N,  
    \end{split}
\end{equation}
where the extended weighted complexity is $\tilde{c_i} = \tilde{z}_i / 2N$.

\subsubsection{Multi-Ouput Weighted Support Vector Machine with Flow Constraints}

Assuming that the analyzed air parcel is sufficiently small so that the flow can be considered approximately incompressible and irrotational, a new set of flow constraints are added to the original set of constraints with the purpose of visualizing the wind velocity field to force the divergence and the vorticity to zero:
\begin{equation}
    \label{eq:flow_constraints}
    \mathrm{s.t.}
    \begin{cases} 
        \left( \tilde{\mathbf{v}}^{k\top}_c \mathbf{\Delta}_{x,y} \mathbf{\dot{V}} \right)  \cdot \left( \tilde{\mathbf{v}}^{k\top}_c \mathbf{\Delta}_{x,y} \mathbf{\dot{V}} \right)^\top &= 0 \\
        \left(  \tilde{\mathbf{v}}^{k\top}_c \mathbf{\Delta}_{x,y} \mathbf{\dot{D}} \right) \cdot \left( \tilde{\mathbf{v}}^{k\top}_c \mathbf{\Delta}_{x,y} \mathbf{\dot{D}} \right)^\top &= 0,
    \end{cases} 
\end{equation}
where the matrices of this expression are defined in Eq. \eqref{eq:matrix_1} Eq. \eqref{eq:set_matrix_1} and Eq. \eqref{eq:set_matrix_2}. To compute the vorticity and divergence, the differentiation of the velocity field along the x-axis, the and y-axis is implemented using operator
\begin{equation}
    \label{eq:matrix_1}
    \mathbf{\Delta}_{x,y} =
    \begin{bmatrix}
        \boldsymbol{\Delta}_x & \mathbf{0} \\
        \mathbf{0} & \boldsymbol{\Delta}_y
    \end{bmatrix}_{2N \times 2N},
\end{equation}
where the differential operators $\boldsymbol{\Delta}_x$ and $\boldsymbol{\Delta}_y$ are defined as,
\begin{equation}
    \label{eq:set_matrix_1}
    \boldsymbol{\Delta}_x =
    \begin{bmatrix}
        -1 & 0 & \ldots & 0\\
        1 & -1 & \ddots & \vdots \\
        0 & 1 & \ddots & 0 \\
        \vdots &  \ddots & \ddots & -1\\
        0 & \ldots & 0 & 1
    \end{bmatrix}_{N \times N}; \quad
    \boldsymbol{\Delta}_y =
    \begin{bmatrix}
        -1 & \ldots & 0 \\
        \vdots & \ddots  & \vdots  \\
        0 & \ldots & -1 \\
        1 & \ldots & 0  \\
        \vdots & \ddots & \vdots \\
        0 & \ldots & 1
    \end{bmatrix}_{N \times N}.
\end{equation}
The operators of the velocity field's vorticity and divergence are respectively,
\begin{equation}
    \label{eq:set_matrix_2}
    \mathbf{\dot{V}} = \left[ \mathbf{I} \quad \mathbf{I} \right]^\top_{2N \times N}, 
    \mathbf{\dot{D}} = \left[ \mathbf{I} \quad -\mathbf{I} \right]^\top_{2N \times N}
\end{equation}

The velocity field is extrapolated to the entire frame using the inferred parameters in frame $k$
\begin{equation}
    \label{eq:extrapolation}
    \hat{\mathbf{v}}^k_c = \left( \tilde{\boldsymbol\alpha}^k_c - \tilde{\boldsymbol\alpha}^{*k}_c \right) \cdot \mathcal{K} \left( \mathbf{X}^{*k}, \mathbf{X} \right) + \mathbf{b}_c^k,
\end{equation}
where the velocity components are $\hat{\mathbf{U}}^k_c \triangleq \hat{\mathbf{v}}^k_{x,c}$, and $\hat{\mathbf{V}}^k_c \triangleq \hat{\mathbf{v}}^k_{y,c}$, where  $\hat{\mathbf{U}}_c^k, \hat{\mathbf{V}}^k_c \in \mathbb{R}^{M \times N} $. 

To compute the flow constraints, the velocity field has to be extrapolated to the whole frame using Eq. \eqref{eq:extrapolation}. The constraints in Eq. \eqref{eq:flow_constraints} are added to the constraints in the dual formulation of the $\varepsilon$-MO-SVM in Eq. \eqref{eq:dual_formaulation}. 
